Byzantine Gathering in Polynomial Time

We study the task of Byzantine gathering in a network modeled as a graph. Despite the presence of Byzantine agents, all the other (good) agents, starting from possibly different nodes and applying the same deterministic algorithm, have to meet at the same node in finite time and stop moving. An adversary chooses the initial nodes of the agents and assigns a different label to each of them. The agents move in synchronous rounds and communicate with each other only when located at the same node. Within the team, f of the agents are Byzantine. A Byzantine agent acts in an unpredictable way: in particular it may forge the label of another agent or create a completely new one. Besides its label, which corresponds to a local knowledge, an agent is assigned some global knowledge GK that is common to all agents. In literature, the Byzantine gathering problem has been analyzed in arbitrary n-node graphs by considering the scenario when GK=(n,f) and the scenario when GK=f. In the first (resp. second) scenario, it has been shown that the minimum number of good agents guaranteeing deterministic gathering of all of them is f+1 (resp. f+2). For both these scenarios, all the existing deterministic algorithms, whether or not they are optimal in terms of required number of good agents, have a time complexity that is exponential in n and L, where L is the largest label belonging to a good agent. In this paper, we seek to design a deterministic solution for Byzantine gathering that makes a concession on the proportion of Byzantine agents within the team, but that offers a significantly lower complexity. We also seek to use a global knowledge whose the length of the binary representation is small. Assuming that the agents are in a strong team i.e., a team in which the number of good agents is at least some prescribed value that is quadratic in f, we give positive and negative results.

==> Sections/onlyfknown.tex <==
\section{Global knowledge $\mathcal{GK}= \lfloor\log \log f\rfloor$}
\label{sec:onlyf}



\subsection{High level idea of the algorithm}\label{subsec:f:gen}

In this section, we aim at solving the $f$-Byzantine gathering problem assuming that $\mathcal{GK}= \lfloor\log \log f\rfloor$. That is, the agents have only an approximated value of $f$. Let $\mathcal{F}_{\min}= 2^{2^{ \lfloor\log \log f\rfloor}}$ and let $\mathcal{F}_{\max}= 2^{(2^{(\lfloor\log \log f\rfloor+1)})}$. Note that $\mathcal{F}_{\min} \leq f < \mathcal{F}_{\max}$, and each agent can compute the same value $\mathcal{F}_{\min}$ and the same value $\mathcal{F}_{\max}$ using $\mathcal{GK}$ . Let $\mathcal{N}$ be a polynomial upper bound on the size of the graph.


In Section~\ref{sec:block}, we introduced subroutine $\swD (\mathcal{D}, \mathcal{N})$,  which solves $f$-Byzantine gathering in polynomial time in $n$ and $\mathcal{D}$ if there are at least $4f+2$ good agents that start executing $\swD (\mathcal{D}, \mathcal{N})$ at the same time from the same node, and the delay between the starting times of $\swD (\mathcal{D}, \mathcal{N})$ by any pair of good agents in the team is at most $\mathcal{D}$. A natural idea, we can come up with in order to guarantee these conditions, would be to require the good agents to execute \sth{\swAA{\mathcal{D}}{\mathcal{N}}{\svX}} (cf. Section~\ref{sec:block}) before executing the aforementioned \sth{\swDD{\mathcal{D}}{\mathcal{N}}}. Indeed, this strategy would turn out to be sucessful if the number of good agents is at least some quadratic polynomial in $f$ and the following conditions are satisfied.

\begin{itemize}
\item The delay between the starting times of $GROUP(\mathcal{D}, \mathcal{N}, bin)$ by any pair of good agents in the team is at most $\mathcal{D}$
\item The set of all the good agents is partitioned into two non empty sets $\mathcal{F}$ (for the set of followers) and $\mathcal{S}$ (for the set of searchers) that execute $GROUP$ with respectively $bin=0$ and $bin=1$.
\item Each agent knows $\mathcal{D}$ and $\mathcal{N}$.
\end{itemize}

Note that, in the case where every agent initially knows $\mathcal{N}$, the first and the third conditions are not really a problem: actually, via the execution of $EXPLO(\mathcal{N})$ we can guarantee that $\mathcal{D}\leq T(EXPLO(\mathcal{N}))$ and that each agent knows this fact. Hence, still in the case where $\mathcal{N}$ is known to all agents, only the second condition is a non-trivial difficulty but it can be tackled using the transformed label of the agents. More precisely, each good agent processes its transformed label bit by bit, and during the process of each bit $b_i$, it executes  $GROUP(\mathcal{D}, \mathcal{N}, b_i)$. So, for any $b_i$, and any pair of good agents, if we keep the delay between the times when these agents start the process of $b_i$ at most $\mathcal{D}\leq T(EXPLO(\mathcal{N}))$ while taking into account some other technicalities, $f$-Byzantine gathering can be eventually achieved in polynomial time in $n$ and $|l_{min}|$. Indeed, this is one of the strategies that is used in Section \ref{sec:onlyn} and in particular via \sth{\swD}. However, $\mathcal{N}$ and $\mathcal{D}$ are initially unknown to every good agent.

One way to circumvent this problem is to make the agents proceed by {steps} $a_1,a_2,a_3,\ldots$ where in each {step} $a_i$, an agent assumes that $\mathcal{N}=2^i$ and  $|l_{\min}| \leq 2^i$ and acts as if the assumption was good. In particular, at the beginning of each {step} $a_i$, an agent can execute $T(EXPLO(2^i))$ in order to make sure that nobody is dormant for the rest of its {step} if $2^i$ upper bounds the size of the graph. Nevertheless, it is worth mentioning that through this strategy, the real delay that has to be taken into account is not only $T(EXPLO(2^i))$: in fact the time to execute {steps} $a_1,a_2,a_3,\ldots,a_{i-1}$ should be added to $T(EXPLO(2^i))$ to obtain this real delay. As a result, such a strategy, which is valid by the way, directly leads to a superpolynomial complexity due to a cumulative effect (at each {step} the supposed cumulative delay has to be multiplied by the number of bits that are processed).

Hence, to achieve our goal, we need to establish a more subtle method. This is the purpose of the rest of this subsubsection. As above, an agent proceeds by {steps} $a_1,a_2,a_3,\ldots$ where in each {step} $a_i$, an agent assumes that $\mathcal{N}=2^i$ and  $|l_{\min}| \leq 2^i$, and acts as if the assumption was good. As above, at the beginning of each {step} $a_i$, an agent executes $T(EXPLO(2^i))$: but the rest of the execution within every {step} is different. Each {step} can be divided into two parts. The aim of the first part is to create a group of at least $4\mathcal{F}_{\max}+2$ {good} agents. Observe that since all the good agents can deduce $\mathcal{F}_{\max}$ from their input, they can detect the creation of such a group {if they are in a group of at least $ 5\mathcal{F}_{\max}+2$  agents}. On another hand, since $f \leq \mathcal{F}_{\max}$, we also ensure the creation of a group of at least $4f+2$ {good} agents.  The aim of the second part is to make sure that all the agents declare the gathering on the same node and at the same round. For this purpose, once a group of at least $4\mathcal{F}_{\max}+2$ {good} agents is created, the good agents of such a group execute subroutine $\sd$ to discover the size of the graph $n$ and deduce the number of rounds they have to wait in order to make sure that every good agent is in a group of at least $4\mathcal{F}_{\max}+2$ {good} agents. The agents can then deduce a polynomial upper bound $\mathcal{D}'$ on $\mathcal{D}$ and execute subroutine $\swD(\mathcal{D}',n)$ to ensure the gathering. 

So, let us focus on the first part that aims at creating a group of at least $4\mathcal{F}_{\max}+2$ {good} agents. While executing the first part of {step} $a_i$ for any positive $i$, the agent assumes that the current hypotheses on $\mathcal{N}$ and $|l_{\min}|$ are true, and it proceeds in two sub-{steps}. During the first sub-{step}, the agent assumes that the maximum delay $\mathcal{D}$ is equal to some predefined polynomial $\mathcal{T}$ which only depends on the current assumptions on $\mathcal{N}$ and $|l_{\min}|$ (it does not take into account the previous actions performed while executing the previous assumptions). It then executes $\swD(\mathcal{T}, 2^i, 2^i)$. If the hypotheses are correct, in view of the properties of $\swD$, we know that all the good agents exit the execution of $\swD$ on the same node and at the same round. In this case, observe that if the number of good agents is at least $2((5f+1)(f+1)+1)$, then when a good agent exits $\swD$, it is in a group on the same node as at least  {$5\mathcal{F}_{\max}+1$} other agents since $\mathcal{F}_{\max}=(\mathcal{F}_{\min})^2$. Thus, our target group is created in this case. That is one of the reasons we will need to assume that the number of good agents is at least $2((5f+1)(f+1)+1)$. By contrast, if one of the hypotheses is not correct, a good agent may not be in a group of at least { $5\mathcal{F}_{\max}+2$} agents when it exits the execution of $\swD$: when this kind of event occurs, it means that either the assumptions of the {step} (on $\mathcal{N}$ and $|l_{\min}|$) are false or $\mathcal{D}>\mathcal{T}$. At this point, the agent keeps trusting the assumptions of $a_i$, and it starts processing the second sub-{step} by assuming that $\mathcal{D}>\mathcal{T}$. Observe that if it is really the case, then we have the following property that is central and crucial for our strategy: the set of all the good agents can be partitioned into two non-empty sets  $\mathcal{G}$ and $\mathcal{G}'$. More precisely, let $\Delta$ be the first round in which a good agent starts the execution of our algorithm. Set $\mathcal{G}$ comprises all the good agents that start the execution of our algorithm by round $t \leq \Delta + \mathcal{T}-1$ while set $\mathcal{G}'$ comprises all the good agents that are not in $\mathcal{G}$. The value of $\mathcal{T}$ has been chosen wisely so that the good agents can have enough time to apply a similar strategy as the one used for \sth{\swA}, i.e. a strategy in which the good agents of one set of the partition will play the role of followers while the good agents of the other set will play the role of searchers. Finally, if the agent finishes the execution of the second sub-{step} without being in a group of at least {$5\mathcal{F}_{\max}+2$} agents, it knows that the assumptions of $a_i$ are false and hence it goes to the next {step} $a_{i+1}$ with new assumptions on $\mathcal{N}$ and $|l_{\min}|$.



%and which ensures the meeting of at least $4f+2$ good agents and then by using  subroutine $\swD$, all the agents exit merge on the same node and at the same round and hence in a node with at least $4\mathcal{F}_{\max}+1$ other agents.




%if the following two conditions are verified: (i) for any pair of good agents, within $\mathcal{D}$ rounds both agents are executing $\swD$.  (ii) At least $4f+2$ good agents start the execution of the subroutine at the same time from the same node. We have also defined subroutine $GROUP(\mathcal{D}, \mathcal{N}, bin)$ which ensures that at least $4f+2$ good agents exit their execution of the subroutine on the same node and at the same round in a time polynomial in $\mathcal{N}$ and $\mathcal{D}$ provided that the following two conditions are verified: (i) for any pair of good agents, within $\mathcal{D}$ rounds both agents are executing $GROUP$. (ii) The set of all the good agents is partitioned into two non empty sets $\mathcal{F}$ (for the set of followers) and $\mathcal{S}$ (for the set of searchers) that execute $GROUP$ with respectively $bin=0$ and $bin=1$.  That is, if we manage to divide the set of the good agents into two subsets $\mathcal{F}$ and $\mathcal{S}$ while preserving a polynomial maximum delay $\mathcal{D}$ then we know how to solve the $f$-Byzantine gathering problem in a polynomial time. 


%One way to obtain sets $\mathcal{F}$ and $\mathcal{S}$ is to use the transformed labels of the agents introduced in Section~\ref{sec:pre}. More precisely, each good agent processes its label bit per bit: during the process of a bit $b_i$, $A$ executes  $GROUP(\mathcal{D}, \mathcal{N}, b_i)$. As each good agent has a unique label, by preserving a maximum polynomial delay $\mathcal{D}$ between each call of $GROUP$, a group of at least $4f+2$ good agents exit their execution of $GROUP$ on the same node and at the same round. Then, by using subroutine $\swD$, the gathering is ensured. This strategy in used in Section \ref{sec:onlyn}. Nevertheless, as in this section, the agents are aware of neither $\mathcal{N}$ nor the length of the smallest label, they have to proceed by making a series of assumptions $a_1, a_2, \dots$ such that in each assumption $a_i$ for any positive integer $i$, agents execute a series of actions $\mathcal{I}$ assuming that $\mathcal{N}=2^i$ and  $|l_{\min}| \leq 2^i$. Since every agent is awakened by either the adversary or any other agent that visits its node, the value of $\mathcal{D}$ depends strongly on the number of rounds a good agent spends executing each previous assumption which also depends on the number of bits each agent processes in each hypothesis. Hence, we cannot use directly the strategy explained above as the gathering will be achieved in an exponential time. As we aim at solving the $f$-Byzantine gathering problem in a polynomial time, to achieve our goal, at each assumption $a_i$ for any positive integer $i$, the agents proceed as follows: the agents first suppose that the maximum delay $\mathcal{D}$ between any pair of agents is equal to some predefined polynomial $\mathcal{T}$, the value of which depends only on the current assumption on $\mathcal{N}$ and $|l_{\min}|$ (it does not take into account the previous actions performed in the previous assumptions). The agents then execute subroutine $\swD(\mathcal{D}, \mathcal{N}, |l_{\min}|)$ presented in section \ref{sec:onlyn}. Assume that assumption $a_i$ is correct. If the assumed delay $\mathcal{D}$ is also correct, in view of the properties of subroutine $\swD$ and $\mathcal{D}$, the gathering is achieved is achieved in a polynomial time. By contrast if the gathering is not achieved then it means that $\mathcal{T}$ is smaller than the actual delay between any pair of agents. Observe that in this case the set of good agents can be partitioned into two sets $\mathcal{G}$ and $\mathcal{G}'$ as explained in the following: let $\Delta$ be the first round in which a good agent starts the execution of our algorithm. Set $\mathcal{G}$ comprises all the good agents that start the execution of our algorithm by round $t \leq \Delta + r\mathcal{T}-1$ where $r$ is some rational number while set $\mathcal{G}'$ comprises all the good agents that are not in $\mathcal{G}$. 


%To explain our strategy, let us first assume that $\mathcal{G}$ is smaller than $\mathcal{G}'$. The idea is to make the agents of $\mathcal{G}$ behave as followers as in subroutine $GROUP$ while the agents of $\mathcal{G}'$ behave as searchers and this during some number $\mathcal{X}$ of rounds chosen in such a way to insure the meeting of at least $5f+2$ agents. More precisely, during the defined $\mathcal{X}$ rounds, the good agents of $\mathcal{G}'$ compute, similarly to \sth{\swA}, an imperfect map $P$ by performing $EXPLO(\mathcal{N})$. Recall that the length of $P$ is the number of visited nodes in $EXPLO(\mathcal{N})$. Let $A$ be the agent computing the map. The $i$-th entry of $P$ of agent $A$ contains a list of couples $(t, \ell_B)$ added for each follower $B$ present on the $i$-th visited node where $t$ is the difference between the number of rounds spent by respectively $A$ and $B$ while executing our algorithm and $\ell_B$ is the label of $B$. This allows $A$ to order the followers met chronologically. The labels are are used to break the symmetry between followers that started the execution of our algorithm simultaneously. The strategy is then similar to the one used in $GROUP$, that is, searcher $A$ moves to the first node $u$ visited during its execution of $EXPLO(\mathcal{N})$ which contains the smallest couple $(t, \ell)$ in $P$ and then it waits on the node reached. The purpose is to make the latest agents move toward the earliest ones. As in GROUP, if $A$ does not see a follower with the label $\ell$ with whom the difference in the number of rounds is $t$, $A$ updates its map by removing $(t, \ell)$ from the list of the $i$-th entry of $P$. That is, in all cases, by choosing the right value of $\mathcal{X}$, a round from which no good searcher updates its map is reached. From such a round, as for $GROUP$, we can show that the total number of different locations that are reached by searchers is at most $f+1$ and then by using the argument of the \emph{pigeonhole principle}, we prove the meeting of at least $5f+2$ agents on some node. Note that since the agents does not know the exact value of $f$, they cannot detect whether there are at least $5f+2$ agents on their node. However, by executing subroutine $\swD$, as the total number of the good agents is at least $2((5f+1)(f+1)+1)> 4\mathcal{F}_{\max}+2$, the agents know that if the gathering occurred then they need to be with at least $4\mathcal{F}_{\max}+1$ other agents when they exit $\swD$. 

%If $\mathcal{G}'$ is larger than $\mathcal{G}$, the agents behave symmetrically. That is the earliest agents move towards the latest ones. More precisely, the agents of $\mathcal{G}$ behave as searcher while the agents of $\mathcal{G}'$ behave as followers. Instead of moving to the first visited node during $EXPLO(\mathcal{N})$ with the smallest couple $(t, \ell)$ in $P$, they move to the first node with the largest couple. In the same manner, we prove that a meeting of at least $5f+2$ agents occurs on some node and then by executing subroutine $\swD$, the agents check whether they are at least $4\mathcal{F}_{\max}+2$ on the same node when they exit $\swD$. 

%Observe that as the agents do not know their number, they cannot declare that the gathering is achieved when they exit $\swD$ on the same node $u$ as at least $4\mathcal{F}_{\max}+1$ other agents.  They need to be sure that every agent is indeed on their current node. As $f \leq \mathcal{F}_{\max}$, the agents know that there are at least $3\mathcal{F}_{\max}+2$ good agents on $u$ and hence they can execute subroutine $\sd$ to compute the size of the graph $n$. Once $n$ is known, $A$ knows how long it has to wait to be sure that every good agent is on the same node as at least $4\mathcal{F}_{\max}+2$ agents. Let $\mathcal{L}$ be the number of rounds for this waiting time. After $\mathcal{L}$ rounds, $A$ executes $\swD$ one more time to make sure that all the groups of at least $4\mathcal{F}_{\max}+2$ meet on the same node and at the round. At this end of this execution, the gathering is declared.

%Two issues remain to be solved: first, the agents are not aware to which group they belong and hence they do not know when to behave as a follower and when to behave as a searcher. To solve this problem all the good agents of both sets $\mathcal{G}$ and $\mathcal{G}'$ execute the same actions so that they behave as searchers and followers for some predefined number of rounds that depends on $\mathcal{T}$, giving time to the good searchers to ensure the meeting of at least $5f+2$ agents. Another problem is, as the agents do not know which of $\mathcal{G}$ and $\mathcal{G}'$ is larger, when a good agent behaves as a searcher, it does not know whether to move to the node that contains the smallest or the largest couple. To solve this second problem, the agents operate in two phases: in the first phase, when a good agent behaves as a searcher, it moves toward the node that contains the smallest couple and in this case the agent first behaves as a searcher and then a follower. When exiting subroutine $\swD$, the agent is not with $4\mathcal{F}_{\max}+1$ other agents, it proceeds by executing the next phase in which it moves toward the node that contains the largest couple and in this case, the agent first behave as a follower and then a searcher. 

	


%Second,  if they behave as a searcher, they do not know whether to move towards the node with the smallest or largest couple. Phases 2 (respectively phase 3) is used to respectively make sure that the gathering is achieved when $\mathcal{G}'$ is larger (respectively when $\mathcal{G}$ is larger). In the second phase, each agent first starts by behaving as a searcher and then a follower to make sure that the agents of $\mathcal{G}$In both phases, each agent behave as a searcher and also a follower during some predefined number of rounds defined using polynomial $\mathcal{T}$ which ensures the the meeting of at least $(5f+2)$ agents. Each of them then executes subroutine $\swD$. 
  
%during the first phase, agents start by behaving as a following for a given number of rounds $x$ and then compute their imperfect map before behaving as searchers for also a given number of rounds. That is, if $\mathcal{G}'$ is larger, then at the right hypothesis, at least $xx$ agents meet on the same node. The agents then perform $\swD$. 
%If the agents did not manage to create a group, then they proceed to phase 3 in which the agent first start behave as a follower and then as a searcher. That is, if in this case, $\mathcal{G}'$ is larger than $\mathcal{G}$, $xx$ agents meet on the same node. And then, as for phase 2, they just have to execute $\swD$. 

%The remaining question is how the good agents can detect whether the gathering has been achieved when they exit subroutine $\swD$. As there at least $(5f+1)(f+1)+1$ good agents, if the gathering is really achieved then at least $4\mathcal{F}_{\max}+2$ agents exit $\swD$ on the same node and at the same rounds. As the agents do not know their number, they cannot declare that the gathering is achieved yet. They need to be sure that every agent is indeed on their current node. For this purpose, the good agents first compute the exact size of the graph by executing \sth{\sd}. Once they discover the size of the graph $n$, they know how long they have to wait to be sure that every good agent is part of a group of at least $4\mathcal{F}_{\max}+2$. Let $\mathcal{T}$ be the number of rounds for this waiting time. After $\mathcal{T}$ rounds the agent execute $\swD$ one more time. At this end of this execution, the gathering is declared.
%	

%Since, the agents do not know the group to which they belong, they do not know whether they should behave as a follower or as a searcher. Moreover, they do not know which of the two groups is larger. These issues are solved in phase 2 and 3. Phase 2 ensures the gathering if set $\mathcal{G}'$ is larger than $\mathcal{G}$ while phase 3 assures the gathering if $\mathcal{G}$ is larger than $\mathcal{G}'$. More precisely, phase 2 makes sure that  the agents first behave as a searcher and then a follower while in phase 3, the agents first behave as a follower and then as a searcher.  By doing so, the agents make sure that a group of at least $4f+2$ agents start the execution of $\swD$ on the same node and at the same round and hence the gathering is then achieved. The strategies used in each of phase 2 and 3 are similar to the strategy used in $GROUP$. That is, the follower remain idle on their nodes during some time to "mark" the position on which a group of at least $4f+2$ agents could meet while the searchers look for these positions. As in subroutine $GROUP$, the searchers compute an imperfect map by performing $EXPLO(\mathcal{N})$. However, instead of associating a visited node $u$ by the list of the followers' labels present on $u$, the searchers also consider the difference in the number of rounds elapsed from the beginning of the execution of our algorithm. That is, the imperfect map of every searcher $A$ is a sequence of lists of couple $(t_A-t_B, \ell_B)$ where $t_A$ (respectively $t_B$) is the number of rounds elapsed from the beginning of the execution of our algorithm for agent $A$ (respectively $B$) and $\ell_B$ is label of the considered follower. By doing so, the searcher can identify, the follower which started.  



\subsection{Formal description of the algorithm}  

We present in this section a deterministic solution for $f$-Byzantine gathering with  $\mathcal{GK}= \lfloor\log \log f\rfloor$.  %Let $\mathcal{F}_{min}= 2^{2^{\lfloor\log \log f\rfloor}}$ and $\mathcal{F}_{max}=2^{2^{\lfloor\log \log f\rfloor}+1}$. Note that $\mathcal{F}_{min} \leq f < \mathcal{F}_{max}$.  
We refer to our algorithm by $\gwn$. Algorithm \ref{onlyf:algo:main} presents the pseudo-code of Algorithm $\gwn$. It calls subroutines $\tc$, $\sd$, $\Syn$, $\cmp$ and $\swD$. %For each agent $A$, we define a predicate variable denoted by $InGroup$. % At any round during the execution of algorithm $\gwn$, if $A$ is on the same node as at least $4\mathcal{F}_{max}+2$ agents, $A$ updates $InGroup$ to true. Otherwise, $InGroup$ is set to false.  
By $T(\tc(i))$ where $i$ is a positive integer, we refer to the maximum number of rounds a good agent can spend executing \stj{\tc(i)}. To ease the description of Algorithm \ref{onlyf:algo:main}, the value of $T({\tc}(i))$, for any positive integer $i$, is given in the description of \stj{\tc(i)}.


\begin{algorithm}
\caption{Algorithm~$\gwn$}
\label{onlyf:algo:main}
\begin{algorithmic}[1]
\State $i \leftarrow 1$
\State $InGroup \leftarrow false$
\While {$\neg (InGroup)$} \label{Test}
	\State Execute $TowerCreation(i)$
	\State $i \leftarrow i+1$ \label{+}
\EndWhile  \label{EndTest}
\State Execute $\sd$   \label{sd}
\State Let $n$ be the value discovered while executing $\sd$

\State $\mathcal{D} \leftarrow  T(\sd) + \sum\limits_{j=1}^{\lceil \log n\rceil +i+3} T({\tc}(j))$ \label{setVariable}
\State Execute $\Syn(\mathcal{D})$ \label{line:Synchro}
\State Execute $\cmp(n)$
\State Let $\mathcal{D}'$ be the value discovered while executing $\cmp(n)$
\State Execute $\swD(\mathcal{D}',n)$  \label{line:A}

\State Declare gathering achieved     \label{line:A+1}
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{Lines \ref{Test} to \ref{EndTest} of Algorithm \ref{onlyf:algo:main} correspond to the first phase of our strategy that aims at creating a group of at least $4\mathcal{F}+2$ agents (refer to Subsection \ref{subsec:f:gen}). When a good agent $A$ executes $\tc(i)$ for any positive integer $i$, $A$ is processing phase $a_i$. Lines \ref{sd} to \ref{line:A+1} correspond to the second part of our strategy explained in Subsection \ref{subsec:f:gen}: it aims at achieving the gathering. For this purpose, agent $A$ first computes the size of the graph $n$ by executing $\sd$. Using the value $n$, by executing subroutines $\Syn$ and $\cmp$, $A$ computes the right value of the maximum delay $\mathcal{D}$ and makes sure that every good agent is in a group of at least $3\mathcal{F}_{\max}+2$ good agents when it starts executing $\swD(\mathcal{D}',n)$.}



Subroutines $\sd$ and $\swDD{\mathcal{D}}{\mathcal{N}}$ are described in Section \ref{sec:pre} and Section \ref{sec:block} respectively. Hence, in this section, we only focus on describing Subroutines $\tc(i)$, $\Syn(i)$ and $\cmp(i)$ for any positive integer $i$.





\subsubsection{\stJ{\tc(i)}}

%During the execution of subroutine ${\tc}(i)$ with $i>0$, agent $A$ assumes that $n \leq 2^{i}$ and $l \leq 2^{i}$. 

While executing $\tc(i)$, a good agent, say $A$, proceeds in three phases: $\del_i$, $\minn_i$ and $\majj_i$. %The index $i$ is omitted when it is clear from the context.  To ease the description of each phase, we assume in the following that during their execution, agent $A$ considers only the agents that are executing the same phase of the same subroutine ${\tc}(i)$ (same parameter). That is, we omit in the following to precise the current phase and the parameter of $\tc$ of the agents.

Before describing the behavior of $A$ in each phase of $\tc(i)$, let us first give some more definitions.

 
By $delay_{(A,B)}$, we denote the time difference $t_A-t_B$ where $t_A$ (respectively $t_B$) is the number of rounds elapsed for agent $A$ (respectively agent $B$) since the beginning of its execution of Algorithm \ref{onlyf:algo:main}. We extend the definition of Function $IM(q,\mathcal{N})$ $(q \in \{0,1\})$ described in Section \ref{sec:block} by adding two more possible values to the parameter $q$, namely $2$ and $3$ (hence $q \in \{0, 1, 2, 3\}$). As when $q \in \{0, 1\}$, the output of $IM(q, \mathcal{N})$ with $q \in \{2, 3\}$, is a sequence $P$ of lists of couples $<L_1, L_2, \dots, L_{T(EXPLO(\mathcal{N}))}>$ that is also called imperfect map. 
Let us explain the behavior of $A$ while executing $IM(2, \mathcal{N})$ (respectively $IM(3, \mathcal{N})$) where $\mathcal{N}$ is equal to $2^i$ for any positive integer $i$ (actually, when $q \in \{2, 3\}$ we will always call the function with a second parameter that is a power of two). Agent $A$ first executes $EXPLO(\mathcal{N})$ with the following additional actions. During the first step, the agent is at the node from which it starts $IM(q, \mathcal{N})$. Let us consider the $j$-{th} step of $EXPLO(\mathcal{N})$ ($j \in \{1, \dots , T(EXPLO(\mathcal{N}))\})$ and let $u$ be the node on which $A$ is at this step. 
If $q=2$ (resp. $q=3$), $L_j$ is a list of pairwise distinct couples $(d, \ell)$ such that $(d, \ell)\in L_j$ iff there is on $u$ an agent $B$ that is (or pretends to be) in \sta{\swY} of phase $\minn_i$ (resp. $\majj_i$) with label $\ell_B=\ell$ and for which $d=delay_{(A,B)}$. \stA{\swY} of phase $\minn_i$ (resp. $\majj_i$) is defined in the formal description of \stj{\tc(i)}. When $(*,\ell_B)$ is added to a list of $P$ by $A$, we say that $A$ records $B$. At the end of $EXPLO(\mathcal{N})$, the agent traverses all the edges traversed in  $EXPLO(\mathcal{N})$ in the reverse order, and then it exits $IM$.

Through the following definition, we present two notions that are similar to that of Definition~\ref{def:index}. The comparisons that are made below among couples of integers follow the classical lexicographic order.

\begin{definition}[Bottom and up index of a map]
\label{def:index-bis}
Let $P=<L_{1}, \dots, L_{T(EXPLO(\mathcal{N})}>$ be a useful map (cf. Definition~\ref{def:use}) computed by Function $IM$ called with a first parameter belonging to $\{2, 3\}$. Let $S$ be the set of every couple that appears in at least one list of $P$. Let $j$ (resp. $j'$) be the smallest integer such that $L_j$ (resp. $L_{j'}$) contains the smallest couple (resp. largest couple) of $S$: $j$ is the bottom index of $P$, while $j'$ is its up index.
\end{definition}

Note that the bottom and up indexes of a map may be equal.

Finally, let us also define an intermediate procedure called $Search(D, N, P, x)$ where $D$ and $N$ are non negative integers, $P$ is a sequence of lists of couples and $x$ is $0$ or $1$.

\paragraph{\stH{Search(D, N, P, x)}.} Let $t$ and $w$ be respectively the round in which $A$ started the execution of $Search(D, N, P, x)$ and a counter initialized to $0$. While $A$ does not reach round $t+ D$, it proceeds as follows:  %if P not useful
Each time $P$ is useful (refer to Definition \ref{def:use}) and $w=0$, $A$ performs the first $(j-1)$ edge traversals of $EXPLO(N)$ from its initial node $v$ where $j$ is the bottom index of $P$ if $x=0$ (respectively the up index of $P$ if $x=1$) : just before each edge traversal, counter $w$ is incremented by one. Let $u$ be the node reached at the end of the $(j-1)$ edge traversals.  {As long as there is an agent $B$ on $u$ in \sta{\swY} of the same phase as $A$ satisfying $delay_{(A,B)}=d$ and $\ell_B=\ell$ where $(d,\ell)$ is the smallest couple if $x=0$ (respectively the largest couple if $x=1$) of the $j$-th list of $P$, $A$ remains idle. By contrast, if there is no such agent on $u$, at some round, if $x=0$ then as long as $y - d \leq \mathcal{D} + T(EXPLO(2^i))$ where $y$ is the number of rounds elapsed for $A$ since the beginning of \sth{Search}, $A$ waits on $u$. For all the remaining cases,  $A$ updates $P$ by removing $(d, \ell)$ from its $j$-th list of $P$ and then goes back to to its initial node $v$ by performing the $(j-1)$ edge traversals executed above in the reverse order: just before each edge traversal of this backtrack, counter $w$ is decremented by one.}

%As long as there is an agent $B$ on $u$ in \sta{\swY} of the same phase as $A$ satisfying $delay_{(A,B)}=d$ and $\ell_B=\ell$ where $(d,\ell)$ is the smallest couple if $x=0$ (respectively the largest couple if $x=1$) of the $j$-th list of $P$, $A$ remains idle. By contrast, if there is no such agent on $u$, at some round, $A$ updates $P$ by removing $(d, \ell)$ from its $j$-th list of $P$ and then goes back to to its initial node $v$ by performing the $(j-1)$ edge traversals executed above in the reverse order: just before each edge traversal of this backtrack, counter $w$ is decremented by one.

As soon as $A$ reaches round $t+D$, if $w=0$ then $A$ exits \sth{Search}. Otherwise, if $w>0$, $A$ goes back to its initial node $v$ by traversing in the reverse order the sequence of $w$ edges $e_1,e_2,\ldots,e_w$ corresponding to the $w$ first edge traversals of $EXPLO(N)$ from node $v$. Once this is done, $A$ exits the procedure.

In all what follows, we set $\mathcal{T}(i) = 4(2^iT(EXPLO(2^i)))^2+ 2T(EXPLO(2^i))$ for any positive integer $i$. We proceed now at the description of each phase of $\tc(i)$. 



\noindent \textbf{Phase} $\del_i$. During this phase, agent $A$ is always in \sta{\szF}. It first performs $EXPLO(2^i)$ and then backtracks it. During this backtrack, if $A$ meets a group of at least {$4\mathcal{F}_{max}+2$} agents having the same indicator (which is defined below in the description of \sth{\Syn}) and executing $\Syn$ at line \ref{line:Synchro} of Algorithm \ref{onlyf:algo:main} with the same parameter $\mathcal{D}$, $A$ interrupts the execution of Phase $\del_i$ and jumps to line \ref{line:Synchro} of Algorithm \ref{onlyf:algo:main} to execute \sth{\Syn} with the same parameter $\mathcal{D}$. By contrast, if $A$ does not meet such a group, it executes \stj{\swBB{2\mathcal{T}(i)}{2^i}{2^i}}. Let $c$ be the round in which $A$ exits Subroutine $\swB$. At round $c$, if $A$ is on a node containing at least {$5\mathcal{F}_{\max}+2$} agents including $A$, all in \sta{\szF} of Phase $\del_i$, $A$ sets $InGroup$ to $true$ and exits $\tc(i)$. Otherwise, $A$ repeats all the actions (edge traversals and waiting periods) performed from the beginning of its execution of $\swBB{2\mathcal{T}(i)}{2^i}{2^i}$ to round $(c-1)$ in the reverse order and then waits $2T(EXPLO(2^i))+2\swBb{2\mathcal{T}(i)}{2^i}{2^i}+T(\sd(2^i))-x$ rounds where $x$ is the number of rounds elapsed from the beginning of Phase $\del_i$. The value of $\swBb{2\mathcal{T}(i)}{2^i}{2^i}$ is given in Section~\ref{sec:onlyn}. At the end of this waiting time, $A$ initiates Phase $\minn_i$ by transiting to \sta{\szG}. 

 %$A$ backtracks $Blackbox$ by performing all its executed actions in the reverse order and then waits $3T(Blackbox(2\mathcal{T}, \mathcal{N}, \ell))-x$ rounds where $x$ is the number of rounds elapsed from the beginning of phase $Delayed$ and $T(Blackbox(2\mathcal{T}, \mathcal{N}, \ell))$ is the maximum number of rounds an agent can spend executing $T(Blackbox(2\mathcal{T}, \mathcal{N}, \ell))$ (refer to section \ref{sec:onlyn}). At the end of this waiting time, $A$ initiates phase $\minn$ by transiting to \sta{\szG}.

\noindent \textbf{Phase} $\minn_i$. During this phase, $A$ can be in one of the following states: \szG{}, \swY{}, \szH{} and \szI{}. At the beginning of this phase, $A$ is in \sta{\szG}. {Let $r_i=\sum\limits_{j=1}^{i-1}T(\tc(j))+T(EXPLO(2^i))$}. The behavior of $A$ for each state is given in the following:
\begin{itemize}

\item \stb{\szG} %Agent $A$ first waits $r_i=\sum\limits_{j=1}^{i-1}T(\tc(j))+T(EXPLO(2^i))$ rounds. At the end of this waiting period, 
Agent $A$ executes $IM(2, 2^i)$ and then transits to \sta{\swY} of Phase $\minn_i$. The output of $IM(2, 2^i)$ is stored in variable $P$. \\ 
% {Note: the initial waiting time of $r_i$ rounds was deleted in \sta{\szG}}

\item \stb{\swY} If $A$ transited to this state from \sta{\szG}, it waits $r_i$ rounds and then transits to \sta{\szH} of Phase $\minn_i$. Otherwise, $A$ waits $r_i$ rounds and then transits to \sta{\szI} of Phase $\minn_i$.  \\

\item \stb{\szH} Agent $A$  first executes $Search(r_i, 2^i, P, 0)$ and then  waits $r_i+ T(EXPLO(2^i))-x$ rounds to transit to \sta{\swY} of Phase $\minn_i$ where $x$ is the number of rounds agent $A$ spent executing $Search(r_i, 2^i, P, 0)$.


\item \stb{\szI{}} Let $z$ be the round in which $A$ started the execution of Subroutine $\minn_i$ and let $z+j$ be the round during the execution of $\minn_i$ in which $A$ is on a node containing the largest number of agents (including agent $A$) such that each of them is either in \sta{\szG}, \swY{} or \szH{} of Phase $\minn_i$. If there are several such rounds, $A$ chooses the one with the largest value of $j$. Agent $A$ repeats exactly the same waiting periods and edge traversals from round $z$ to round $z+j-1$ and then it executes Subroutine $\swD ({\mathcal{R}_i+r_i}, 2^i)$ where {$\mathcal{R}_i = 3r_i+3T(EXPLO(2^i))$}. Let $c$ be the round in which $A$ exits Subroutine $\swD$. At round $c$, if $A$ is on a node containing at least  {$5\mathcal{F}_{\max}+2$} agents including $A$, all in \sta{\szI} of Phase $\minn_i$, $A$ sets $InGroup$ to $true$ and exits Subroutine $\tc(i)$. Otherwise, $A$ repeats all the actions (edge traversals and waiting periods) performed from the beginning of Phase $\minn_i$ to round $(c-1)$ in the reverse order and then waits $2(2\mathcal{R}_i+ T(\swD ({\mathcal{R}_i+r_i}, 2^i))-x$ rounds where $x$ is the number of rounds elapsed from the beginning of $\minn_i$. The value of $T(\swD ({\mathcal{R}_i+r_i}, 2^i))$ is given in Section \ref{sec:block}. At the end of this waiting time, $A$ transits to \sta{\swY} of Phase $\majj_i$. 

\end{itemize}

\noindent  \textbf{Phase} $\majj_i$. During this phase, $A$ can be in one of the following states: \swY{}, \szH{} and \szI{}. Although we use the same names of states as in Subroutine $\minn_i$, the behavior of $A$ is different as explained in the sequel. At the beginning of this phase, $A$ is in \sta{\swY}.

\begin{itemize}

\item \stb{\swY} Agents $A$ waits on its current node $r_i+ 2T(EXPLO(2^i))+2\mathcal{T}(i)$ rounds and then transits to \sta{\szH} of Phase $\majj_s$.

\item \stb{\szH} Agent $A$ first executes $IM(3, 2^i)$. The output of this execution is stored in variable $P$. Next, it executes $Search(r_i, 2^i, P, 1)$ and then waits $r_i+T(EXPLO(2^i))-x$ rounds to transit to \sta{\szI} of Phase $\majj_i$ where $x$ is the number of rounds $A$ spent executing $Search(r_i, 2^i, P, 1)$.


\item \stb{\szI} Let $z$ be the round in which $A$ started the execution of Subroutine $\majj_i$ and let $z+j$ be the round during the execution of $\majj_i$ in which $A$ is on a node containing the largest number of agents (including agent $A$) such that each of them is either in \sta{\swY} or in \sta{\szH} of Phase $\majj_i$. If there are several such rounds, $A$ chooses the one with the largest value of $j$. Agent $A$ repeats exactly the same waiting periods and edge traversals from round $z$ to round $z+j-1$ and then it executes $\swD ( {\mathcal{R}'_i+ r_i}, 2^i)$ where $\mathcal{R}_i' = 2r_i+5T(EXPLO(2^i))+2\mathcal{T}(i)$. Let $c$ be the round in which $A$ exits $\swD$.
 At round $c$, if $A$ is on a node containing at least {$5\mathcal{F}_{\max}+2$} agents including $A$, all in \sta{\szI} of Phase $\majj_i$, $A$ sets $InGroup$ to $true$ and exits $\tc(i)$. Otherwise,  $A$ repeats all the actions (edge traversals and waiting periods) performed from the beginning of Phase $\majj$ to round $(c-1)$ in the reverse order and then waits $2(2\mathcal{R}'_i+T(\swD ( {\mathcal{R}'_i+r_i}, 2^i)))-x$ rounds where $x$ is the number of rounds elapsed from the beginning of $\majj_i$. The value of $T(\swD ( 2\mathcal{R}'_i, 2^i))$ is given in Section \ref{sec:block}. At the end of this waiting time, $A$ exits $\tc(i)$. 
\end{itemize}

Let $T(\del_i)$, $T(\minn_i)$ and $T(\majj_i)$ be the maximum number of rounds a good agent can spend in respectively Phase $\del_i$, $\minn_i$ and $\majj_i$. For any positive integer $i$, $T(\tc(i))= T(\del_i)+ T(\minn_i) + T(\majj_i)$.

%\subsubsection{\stH{\sd}}
%
%Let $A$ be a good agent executing $\sd$ and let $u$ be the node of $A$ at the beginning of this execution. The aim for $A$ is to discover the value of $n$.  When $A$ starts the execution of $\sd$, it is in \sta{\szM}. Beside its state, $A$ transmits its label to the agents being on node $u$. It assigns to variable $L$ the list of all pairwise distinct labels of the agents in \sta{\szM} on $u$, in the increasing order. We call $L$, the group label of $A$. If $\ell_A$, the label of agent $A$, is among the first half of $L$, then $A$ executes \sth{EST} as the explorer in $EST$. Otherwise, it executes $EST$ as the stationary token in $EST$. Recall that during the execution of $EST$, if $A$ is an explorer, $A$ constructs a $BFS$ tree rooted at its starting node $u$ marked by the stationary token \cite{ChalopinDK10}. In the beginning of $EST$, $A$ adds the root $u$ to the tree and then it makes the process of $u$. The process of a node $w$ consists in checking all the neighbors of $w$ in order to determine whether some of them
%have to be added to the tree or not. While executing $EST$, if $A$ is an explorer then it considers as its stationary token any group of at least $\mathcal{F}_{max}+1$ agents with the same group label $L$ executing $EST$ as a stationary token. When $A$ becomes aware of the value of the size of the graph $n$, $A$ returns to its initial node $u$ and informs the agents on $u$ of the value of $n$ and then it exits subroutine $\sd$ by returning the value of $n$. Similarly, if $A$ is a stationary token then $A$ considers as its explorer any group of at least $\mathcal{F}_{max}+1$ agents sharing the same group label $L$ and executing $EST$ as explorers. When the group of explorers returns to node $u$ with the final value of $n$, $A$ exits subroutine $\sd$ by returning the value of $n$. 


\subsubsection{Subroutine: ${\Syn}(i)$}

When $A$ starts executing ${\Syn(i)}$, it enters \sta{\szJ}. From the description of our algorithm, $A$ can either enter \sta{\szJ} after executing line \ref{setVariable} of Algorithm \ref{onlyf:algo:main} or from Phase $\del_j$ for any positive integer $j$.  In both cases, we assume that in each round within the execution of ${\Syn}(i)$, agent $A$ tells the other agents sharing the same node an indicator described below.

When agent $A$ enters \sta{\szJ} of ${\Syn(i)}$ after executing line \ref{setVariable} of Algorithm \ref{onlyf:algo:main}, $A$ waits $i$ rounds and then exits \sth{\Syn(i)}. In each round within the execution of ${\Syn}(i)$, the indicator of $A$ is a couple $(t,n)$ where $t$ is the number of rounds elapsed from the beginning of the execution of $\Syn(i)$ (including the current one) by agent $A$, and $n$ is the graph size that it discovered when executing $\sd$ (cf. line \ref{setVariable} of Algorithm \ref{onlyf:algo:main}).

When $A$ enters \sta{\szJ} from Phase $\del_j$, in the previous round, it met a group of at least {$4\mathcal{F}_{max}+2$} agents having the same indicator $(t',n')$. While in this state, agent $A$ waits $i-t'$ rounds and then exits \sth{\Syn(i)}. In each round spent in this state, the indicator of $A$ is $(i-t'+r,n')$ where 
$r$ is the number of rounds elapsed from the beginning of the execution of $\Syn(i)$ (including the current one) by agent $A$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ù
\subsubsection{Subroutine $\cmp(i)$}

During the execution of Subroutine $\cmp(i)$, agent $A$ can be either in \sta{\szK} or \szL{}. When $A$ starts executing $\cmp(i)$, it enters \sta{\szK}. In each round within the execution of $\cmp(i)$, $A$ tells the other agents sharing the same node an integer called mark {which is the value of the parameter of Subroutine $\Syn$ executed by $A$ previously}.

\noindent \stb{\szK} Agent $A$ assigns to variable $H$ the list of all pairwise distinct labels of the agents which are also in \sta{\szK} on the same node. Agent $A$ then transits to \sta{\szL}. \\

\noindent \stb{\szL} When $A$ enters this state, it assigns $0$ to $\mathcal{D}'$ and initializes an array $\mathcal{P}$ of size $T(EXPLO(n))$: each entry of $\mathcal{P}$ is a list of integers that is initially empty. 

If $\ell_A$ belongs to the first $\lceil \frac{H}{2}\rceil$ labels of $H$, $A$ performs $EXPLO(i)$ and then backtracks it. At the $j$-th round of $EXPLO(i)$ (for all $1\leq j\leq T(EXPLO(i))$, if $A$ meets a group of at least $3\mathcal{F}_{\max}+2$ agents executing $\swD(\mathcal{X}, i)$ of line \ref{line:A} of Algorithm \ref{onlyf:algo:main}, $A$ sets $\mathcal{D}'=\mathcal{X}$. 
{If it meets a group of at least $3\mathcal{F}_{\max}+2$ agents in \sta{\szJ} executing $\Syn(\mathcal{J})$ and sharing the same indicator $(t,i)$, $A$ adds $\mathcal{J}$ to the list $\mathcal{P}[j]$. Finally, if $A$ meets a group of at least $\mathcal{F}_{\max}+1$ agents in either \sta{\szL} or \szK{} sharing the same mark $\alpha$, $A$ adds $\alpha$ to the list $\mathcal{P}[j]$.  At the end of the backtrack, if $\mathcal{D}'=0$, $A$ sets $\mathcal{D}'$ to the following value: $\max\{\mathcal{P}[k], \forall k \in [1,T(EXPLO(i))]\}$. %(Informally speaking $D'$ corresponds to the maximal delay between the starting times of the executions of \sth{\Syn} by two groups of agents having finished to execute \sth{\sd}). 
It then waits one round to exit Subroutine $\cmp(i)$.}





%If it meets a group of at least $3\mathcal{F}_{\max}+2$ agents in \sta{\szJ} sharing the same indicator $(t,i)$, $A$ adds $t-\mathcal{J}$ to the list $\mathcal{P}[j]$. Finally, if $A$ meets a group of at least $\mathcal{F}_{\max}+1$ agents in either \sta{\szL} or \szK{} sharing the same mark $\alpha$, $A$ adds $\alpha$ to the list $\mathcal{P}[j]$. At the end of the backtrack, if $\mathcal{D}'=0$, $A$ sets $\mathcal{D}'$ to the following value:\\
%$\max\{(|(x_k-k)-(x_k'-k')|), \forall k,k'\in \{1,T(EXPLO(i))\}\mbox{ }and\mbox{ }\forall x_k (resp.\mbox{ }x_{k'}) \in P[k] (resp.\mbox{ }P[k'])\}$. (Informally speaking $D'$ corresponds to the maximal delay between the starting times of the executions of \sth{\Syn} by two groups of agents having finished to execute \sth{\sd}). It then waits one round to exit subroutine $\cmp(i)$.

If $\ell_A$ does not belong to the first $\lceil \frac{H}{2}\rceil$ labels of $H$, $A$ waits $2T(EXPLO(i))+1$ rounds on its current node. At the end of this waiting time, $A$ assigns to its variable $\mathcal{D}'$, the value of $\mathcal{D}'$ shared by at least $\mathcal{F}_{\max}+1$ agents, the labels of which belong to the first $\lceil \frac{H}{2}\rceil$ labels of $H$. Agent $A$ then exits Subroutine $\cmp(i)$.


 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Correctness and complexity analysis}

% {Note: The definition of set $\mathcal{E}$ along with all its occurrences were deleted}.
 
Let $\Delta$ be the first round in which a good agent starts executing Algorithm \ref{onlyf:algo:main}.  By initial node of a given good agent $A$, we refer to the node from which $A$ starts executing Algorithm \ref{onlyf:algo:main}. In the rest  of this proof, we assume that the {total} number of good agents is at least $2((5f+1)(f+1)+1)$.

We start with the following proposition that directly follows from the description of the algorithm. 

\begin{proposition}\label{pro:delayed}
Let $A$ be a good agent that starts executing $\tc(i)$ for any positive integer $i$. The following three properties hold.
\begin{itemize}

\item If $A$ finishes the execution of $\del_i$ without setting its variable $InGroup$ to $true$ then $A$ has spent exactly $T(\del_i)=2T(EXPLO(2^i))+2T(\swD({2\mathcal{T}(i)}, 2^i, 2^i))+T(\sd(2^i))$ rounds executing Phase $\del_i$. Moreover, $A$ finishes the execution of $\del_i$ on its initial node.
\item If $A$ finishes the execution of $\minn_i$ without setting its variable $InGroup$ to $true$ then $A$ has spent exactly $T(\minn_i)= 2(2\mathcal{R}_i+ T({\swD(\mathcal{R}_i+r_i}, 2^i)))$ rounds executing Phase $\minn_i$. Moreover, $A$ finishes the execution of $\minn_i$ on its initial node.
\item If $A$ finishes the execution of $\majj_i$ without setting its variable $InGroup$ to $true$ then $A$ has spent exactly $T(\majj_i)=2(2\mathcal{R}'_i+ T(\swD({\mathcal{R}'_i+r_i}, 2^i)))$ rounds executing Phase $\majj_i$. Moreover, $A$ finishes the execution of $\majj_i$ on its initial node.
\end{itemize}
  
\end{proposition}


%\begin{lemma}\label{f:lemma:delay1}
%Let $A$ be a good agent which is executing phase $\del_i$ for any positive integer $i$. If $A$ finishes the execution of $\del_i$ without setting its $InGroup$ to $true$ then $A$ has spent exactly $T(\del_i)=2T(EXPLO(2^i))+2T(\swD(2\mathcal{T}(i), 2^i, 2^i))$ rounds executing phase $\del_i$
%\end{lemma}
%
%\begin{proof}
%When $A$ starts the execution of phase $\del_i$, it first spends $2T(EXPLO(2^i))$ rounds performing $EXPLO(2^i)$ and then backtracking it. Since by assumption, $A$ executes phase $\minn_i$, at the end of the backtrack,  $A$ executes $\swD(2\mathcal{T}(i), 2^i, 2^i)$ which lasts at most $T(\swD(2\mathcal{T}(i), 2^i, 2^i))$ rounds (refer to section \ref{sec:onlyn}). Let $c$ be the round in which $A$ exits $\swD$. Again since by assumption $A$ executes phase $\minn_i$, it repeats all the edge traversals and waiting procedure performed from the beginning of phase $\swD(2\mathcal{T}(i), 2^i, 2^i)$ to round $(c-1)$ in the reverse order and then waits  $2T(EXPLO(2^i))+2T(\swD(2\mathcal{T}(i), 2^i, 2^i))-x$ rounds where $x$ is the number of rounds elapsed from the beginning of phase $\del_i$. Observe that $x \leq 2T(EXPLO(2^i))+2T(\swD(2\mathcal{T}(i), 2^i, 2^i))$. Hence, we can deduce that $A$ spends exactly $T(\del_i)=2T(EXPLO(2^i))+2T(\swD(2\mathcal{T}(i), 2^i, 2^i))$ rounds executing phase $\del_i$.
%\end{proof}
%
%\begin{lemma}\label{f:lemma:delay2}
%Let $A$ be a good agent which is executing phase $\minn_i$ for any positive integer $i$. If $A$ finishes the execution of $\minn_i$ without setting its $InGroup$ to $true$ then $A$ has spent exactly $T(\minn_i)= 2(\mathcal{R}_i+ T(\swD(2\mathcal{R}, 2^i)))$ rounds executing phase $\minn_i$ rounds executing phase $\minn_i$
%\end{lemma}
%
%\begin{proof}
%Let $t$ be the round in which $A$ starts the execution of phase $\minn_i$. From the algorithm, agent $A$ is in \sta{\szG} at round $t$. While in \sta{\szG}, $A$ first waits $r_i=\sum\limits_{j=1}^{i-1} \tc(j)+T(EXPLO(2^i))$ rounds and then performs $IM(2, 2^i)$ that lasts $2T(EXPLO(2^i))$ rounds before transiting to \sta{\swY} of phase $\minn_i$. While in \sta{\swY}, $A$ waits $r_i$ rounds and then transits  to \sta{\szH} of its current phase. Agent $A$ then remains in \sta{\szH} for $m$ rounds where $r_i \leq m \leq r_i+T(EXPLO(2^i))$. Then, it transits again to \sta{\swY} in which it spends $r_i$ rounds before transiting to \sta{\szI} of phase $\minn_i$. When $A$ transits to \sta{\szI}, $A$ has spent at most $\mathcal{R}_i=4r_i+3T(EXPLO(2^i))$ rounds in phase $\minn_i$. Moreover, $A$ is on its initial node (refer to the description of \sta{\szH}). Let $t'$ be the round in which $A$ enters \sta{\szI} of phase $\minn_i$. Agent $A$ repeats the same waiting periods and edge traversals executed from round $t$ to some given round $t+\beta < t'$ before executing $\swD(2\mathcal{R}_i, 2^i)$ which lasts $T(\swD(2\mathcal{R}_i, 2^i))$ rounds (refer to section \ref{sec:block}). When $A$ exits $\swD(2\mathcal{R}_i, 2^i)$, since $A$ does not set its $InGroup$ predicate to $true$ by assumption, it repeats all the waiting periods and edge traversals performed from the beginning of phase $\minn_i$ in the reverse order and then waits $2(\mathcal{R}_i+ T(\swD(2\mathcal{R}, 2^i)))-x$ rounds before starting phase $\majj_i$ where $x$ is the number of rounds elapsed from the beginning of phase $\minn_i$. Observe that $x \leq 2(\mathcal{R}_i+ T(\swD(2\mathcal{R}, 2^i)))$. We can hence deduce that $A$ spends exactly $T(\minn_i)= 2(\mathcal{R}_i+ T(\swD(2\mathcal{R}, 2^i)))$ rounds executing phase $\minn_i$.
%\end{proof}
%
%\begin{lemma}\label{f:lemma:delay3}
%Let $A$ be a good agent which is executing phase $\minn_i$ for any positive integer $i$. If $A$ finishes the execution of $\majj_i$ without setting its $InGroup$ to $true$ then $A$ has spent exactly $T(\majj_i)=2(\mathcal{R}'_i+ T(\swD(2\mathcal{R}', 2^i)))$ rounds executing phase $\majj_i$
%\end{lemma}
%
%\begin{proof}
%$\majj_i$. Let $t$ be the round in which $A$ starts the execution of phase $\majj_i$. From the algorithm, $A$ first spends $r_i+2T(EXPLO(2^i))+2\mathcal{T}(i)$ rounds in \sta{\swY} of phase $\majj_i$ before performing $IM(3,2^i)$ which lasts $2T(EXPLO(2^i))$ rounds. Agent $A$ then transits to \sta{\szH} of its current phase in which it remains $m$ rounds where $r_i \leq m \leq r_i+T(EXPLO(2^i))$. Then, it transits to \sta{\szI} of phase $\majj_i$. Let $t'$ be the round in which $A$ enters \sta{\szI}. At round $t'$, $A$  has spent at most $\mathcal{R}'=2r_i+5T(EXPLO(2^i))+2\mathcal{T}(i)$ rounds executing $\majj_i$. Moreover, $A$ is on its initial node (refer to the description of \sta{\szH} of phase $\majj_i$). Let $t'$ be the round in which $A$ enters \sta{\szI} of phase $\majj_i$. Agent $A$ repeats the same waiting periods and edge traversals executed from round $t$ to some given round $t+\beta < t'$ before executing $\swD(2\mathcal{R}'_i, 2^i)$ which lasts $T(\swD(2\mathcal{R}_i, 2^i))$ rounds (refer to section \ref{sec:block}). When $A$ exits $\swD(2\mathcal{R}_i, 2^i)$, since $A$ does not set its $InGroup$ variable to true, it repeats all the waiting periods and edge traversals performed from the beginning of phase $\majj_i$ in the reverse order and then waits $2(\mathcal{R}'+T(\swD(2\mathcal{R}_i, 2^i)))-x$ rounds before exiting subroutine $\tc(i)$ where $x$ is the number of rounds elapsed from the beginning of phase $\majj_i$. Observe that $x \leq 2T(\minn_i)$. We can hence deduce that $A$ spends exactly $T(\majj_i)=2(\mathcal{R}'_i+T(\swD(2\mathcal{R}_i, 2^i)))$ rounds executing phase $\majj_i$.
%\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lemma}\label{f:lemma:delay}
%Let $A$ be a good agent which is executing $\tc(i)$ for any positive integer $i$. If $A$ exits $\tc(i)$ with its $InGroup$ set to $false$ then $A$ has spent exactly:
%\begin{enumerate}
%\item $T(\del_i)=2T(EXPLO(2^i))+2T(\swD(2\mathcal{T}(i), 2^i, 2^i))$ rounds executing phase $\del_i$
%\item $T(\minn_i)= 2(\mathcal{R}_i+ T(\swD(2\mathcal{R}, 2^i)))$ rounds executing phase $\minn_i$.
%\item $T(\majj_i)=2(\mathcal{R}'_i+ T(\swD(2\mathcal{R}', 2^i)))$ rounds executing phase $\majj_i$. 
%\end{enumerate}
%
%\end{lemma}
%
%\begin{proof}
%Since $A$ exits $\tc(i)$ with its $InGroup$ set to $false$, $A$ executes every phase of subroutine $\tc(i)$ (refer to the description of $\tc(i)$). Let us consider the number of rounds spent in each phase of $\tc(i)$ separately:
%	\begin{enumerate}
%	\item Phase $\del_i$. When $A$ starts the execution of phase $\del_i$, it first spends $2T(EXPLO(2^i))$ rounds performing $EXPLO(2^i)$ and then backtracking it. Since by assumption, $A$ executes phase $\minn_i$, at the end of the backtrack,  $A$ executes $\swD(2\mathcal{T}(i), 2^i, 2^i)$ which lasts at most $T(\swD(2\mathcal{T}(i), 2^i, 2^i))$ rounds (refer to section \ref{sec:onlyn}). Let $c$ be the round in which $A$ exits $\swD$. Again since by assumption $A$ executes phase $\minn_i$, it repeats all the edge traversals and waiting procedure performed from the beginning of phase $\swD(2\mathcal{T}(i), 2^i, 2^i)$ to round $(c-1)$ in the reverse order and then waits  $2T(EXPLO(2^i))+2T(\swD(2\mathcal{T}(i), 2^i, 2^i))-x$ rounds where $x$ is the number of rounds elapsed from the beginning of phase $\del_i$. Observe that $x \leq 2T(EXPLO(2^i))+2T(\swD(2\mathcal{T}(i), 2^i, 2^i))$. Hence, we can deduce that $A$ spends exactly $T(\del_i)=2T(EXPLO(2^i))+2T(\swD(2\mathcal{T}(i), 2^i, 2^i))$ rounds executing phase $\del_i$ in this case.
%	
%	\item Phase $\minn_i$. Let $t$ be the round in which $A$ starts the execution of phase $\minn_i$. From the algorithm, agent $A$ is in \sta{\szG} at round $t$. While in \sta{\szG}, $A$ first waits $r_i=\sum\limits_{j=1}^{i-1} \tc(j)+T(EXPLO(2^i))$ rounds and then performs $IM(2, 2^i)$ that lasts $2T(EXPLO(2^i))$ rounds before transiting to \sta{\swY} of phase $\minn_i$. While in \sta{\swY}, $A$ waits $r_i$ rounds and then transits  to \sta{\szH} of its current phase. Agent $A$ then remains in \sta{\szH} for $m$ rounds where $r_i \leq m \leq r_i+T(EXPLO(2^i))$. Then, it transits again to \sta{\swY} in which it spends $r_i$ rounds before transiting to \sta{\szI} of phase $\minn_i$. When $A$ transits to \sta{\szI}, $A$ has spent at most $\mathcal{R}_i=4r_i+3T(EXPLO(2^i))$ rounds in phase $\minn_i$. Moreover, $A$ is on its initial node (refer to the description of \sta{\szH}). Let $t'$ be the round in which $A$ enters \sta{\szI} of phase $\minn_i$. Agent $A$ repeats the same waiting periods and edge traversals executed from round $t$ to some given round $t+\beta < t'$ before executing $\swD(2\mathcal{R}_i, 2^i)$ which lasts $T(\swD(2\mathcal{R}_i, 2^i))$ rounds (refer to section \ref{sec:block}). When $A$ exits $\swD(2\mathcal{R}_i, 2^i)$, since $A$ does not set its $InGroup$ predicate to $true$ by assumption, it repeats all the waiting periods and edge traversals performed from the beginning of phase $\minn_i$ in the reverse order and then waits $2(\mathcal{R}_i+ T(\swD(2\mathcal{R}, 2^i)))-x$ rounds before starting phase $\majj_i$ where $x$ is the number of rounds elapsed from the beginning of phase $\minn_i$. Observe that $x \leq 2(\mathcal{R}_i+ T(\swD(2\mathcal{R}, 2^i)))$. We can hence deduce that $A$ spends exactly $T(\minn_i)= 2(\mathcal{R}_i+ T(\swD(2\mathcal{R}, 2^i)))$ rounds executing phase $\minn_i$.
%	
%	\item Phase $\majj_i$. Let $t$ be the round in which $A$ starts the execution of phase $\majj_i$. From the algorithm, $A$ first spends $r_i+2T(EXPLO(2^i))+2\mathcal{T}(i)$ rounds in \sta{\swY} of phase $\majj_i$ before performing $IM(3,2^i)$ which lasts $2T(EXPLO(2^i))$ rounds. Agent $A$ then transits to \sta{\szH} of its current phase in which it remains $m$ rounds where $r_i \leq m \leq r_i+T(EXPLO(2^i))$. Then, it transits to \sta{\szI} of phase $\majj_i$. Let $t'$ be the round in which $A$ enters \sta{\szI}. At round $t'$, $A$  has spent at most $\mathcal{R}'=2r_i+5T(EXPLO(2^i))+2\mathcal{T}(i)$ rounds executing $\majj_i$. Moreover, $A$ is on its initial node (refer to the description of \sta{\szH} of phase $\majj_i$). Let $t'$ be the round in which $A$ enters \sta{\szI} of phase $\majj_i$. Agent $A$ repeats the same waiting periods and edge traversals executed from round $t$ to some given round $t+\beta < t'$ before executing $\swD(2\mathcal{R}'_i, 2^i)$ which lasts $T(\swD(2\mathcal{R}_i, 2^i))$ rounds (refer to section \ref{sec:block}). When $A$ exits $\swD(2\mathcal{R}_i, 2^i)$, since $A$ does not set its $InGroup$ variable to true, it repeats all the waiting periods and edge traversals performed from the beginning of phase $\majj_i$ in the reverse order and then waits $2(\mathcal{R}'+T(\swD(2\mathcal{R}_i, 2^i)))-x$ rounds before exiting subroutine $\tc(i)$ where $x$ is the number of rounds elapsed from the beginning of phase $\majj_i$. Observe that $x \leq 2T(\minn_i)$. We can hence deduce that $A$ spends exactly $T(\majj_i)=2(\mathcal{R}'_i+T(\swD(2\mathcal{R}_i, 2^i)))$ rounds executing phase $\majj_i$.
%	\end{enumerate}
%	
%	From the three cases above we can deduce that the lemma holds.   
%\end{proof}

From Proposition \ref{pro:delayed}, we get the following corollaries.

\begin{corollary}\label{onlyf:timetc}
For any positive integer $i$, if $A$ exits Subroutine $\tc(i)$  with $InGroup=false$ then $A$ has spent exactly $T(\tc(i))=T(\del_i)+T(\minn_i)+T(\majj_i)$ rounds executing Subroutine $\tc(i)$.  
\end{corollary}

\begin{corollary}\label{each-phase}
Let $A$ and $B$ be any good agents such that $delay_{(A,B)} \geq 0$. For any positive integer $i$, if both $A$ and $B$ exit $\tc(i)$ with their respective $InGroup$ set to false then $A$ starts executing $\tc(i+1)$ from its initial node exactly $delay_{(A,B)}$ rounds before $B$.  
\end{corollary}

Let $s$ be the smallest positive integer verifying $\max(n, |l_{\min}|) \leq 2^s$. We define round $\Delta_s$ to be the first round (if any) at which a good agent starts the execution of $\tc(s)$. 

%Let us first assume that for any good agent $A$ and $0< i <s$, $A$ does not exit subroutine $\tc(i)$  with its $InGroup$ equal to $true$. From algorithm \ref{onlyf:algo:main} (from line \ref{Test} to line \ref{+}) and corollary \ref{onlyf:timetc}, $A$ executes $\tc(s)$ after $\sum \limits_{j=0}^{s-1} T(\tc(j))$ rounds after its Wake up. 

\begin{lemma}\label{f:lemma:awake}
If there is a good agent $A$ that executes $\tc(s)$ then every good agent is awake at round $\Delta_s+T(EXPLO(2^s)$.
\end{lemma}

\begin{proof}
Let $A$ be a good agent which starts the execution of $\tc(s)$ at round $\Delta_s$. At round $\Delta_s$, $A$ starts executing Phase $\del_s$. However, the beginning of Phase $\del_s$ consists in executing $EXPLO(2^s)$ first. Since $n \leq 2^s$, $A$ visits every node of the graph at least once. Thus, the lemma holds. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}  \label{f:lemma:maxdelay}
For any pair of good agents $A$ and $B$, $|delay_{(A,B)}| \leq r_s$.
% T(EXPLO(2^s))+\sum\limits_{j=1}^{s-1} \tc(j)$.
\end{lemma}

\begin{proof}

By lemma \ref{f:lemma:awake}, at round $\Delta_s+T(EXPLO(2^s))$, every good agent is awake. Let $B$ be the last good agent to wake-up. Agent $B$ starts the execution of Algorithm \ref{onlyf:algo:main} at round $t=\Delta_s+T(EXPLO(2^s))$ at the latest. As the earliest good agent has spent at most $T(EXPLO(2^s))+\sum\limits_{j=1}^{s-1} \tc(j)$ rounds executing Algorithm~\ref{onlyf:algo:main}, the claim holds.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


\begin{lemma}\label{f:lemma:del}
If every good agent $A$ starts the execution of Phase $\del_s$ by round {$\Delta_s + 2\mathcal{T}(s)-1$} then all the good agents exit $\tc(s)$ with their $InGroup= true$ in the same node and at the same round $ t < \Delta_s + T(\del_s)$.
%least ($4\mathcal{F}_{max}+2$) good agents exit $\tc(s)$ from the same node and at the same round $ t < \Delta_s + T(\del_s)$.
\end{lemma}

\begin{proof}
When a good agent $A$ executes Phase $\del_s$, it first performs $T(EXPLO(2^s))$ and then backtracks it. Since by assumption every good agent starts the execution of phase $\del_s$ by round {$\Delta_s + 2\mathcal{T}(s)-1$}, $A$ starts executing {$\swD(2\mathcal{T}(s), 2^s, 2^s)$} between round $\Delta_s+2T(EXPLO(2^s))$ and round {$\Delta_s+2\mathcal{T}(s)+2T(EXPLO(2^s))-1$}. As the {total} number of good agents is at least $2 ((5f+1)(f+1)+1)$, by Theorem \ref{onlyn:proof:live}, we know that all good agents exit {$\swD(2\mathcal{T}(s), 2^s, 2^s)$} on the same node and at the same round {$t \leq \Delta_s + 2T(EXPLO(2^s))+ T(\swD(2\mathcal{T}(s), 2^s, 2^s))$}. Remember that $f\geq \mathcal{F}_{\min}=2^{2^{\lfloor\log \log f\rfloor}}$.  As $\mathcal{F}_{max}=(\mathcal{F}_{min})^2$, we have $2((5 \mathcal{F}_{min}+1) (\mathcal{F}_{min}+1)+1) \geq 4\mathcal{F}_{max}+2$ which means that there are at least $4\mathcal{F}_{max}+2$ good agents. From the description of phase $\del_s$, when at least $4\mathcal{F}_{max}+2$ good agents exit $\swD(4\mathcal{T}(s), 2^s, 2^s)$ on the same node and the same round, each of them sets its variable $InGroup$ to $true$ and also exits $\tc(s)$. This proves the lemma.
\end{proof}

Let $\mathcal{G}_1$ and $\mathcal{G}_2$ be two sets of good agents defined as follows: a good agent $A$ is in $\mathcal{G}_1$ if $A$ starts the execution of $\del_s$ by round {$\Delta_s + \mathcal{T}(s)-1$}. Set $\mathcal{G}_2$ {contains} every good agent which is not in $\mathcal{G}_1$. %Unless stated otherwise, we assume in all what follows that $|\mathcal{G}_2|\ne \emptyset$. 


\begin{lemma}\label{f:lemma:minn}
%A group of at least $4\mathcal{F}_{max}+2$ good agents exit $\tc(s)$ on the same node and at the same round $t <  \Delta_s + T(\del_s) + T(\minn_s)$ if the following two conditions are verified:
All the good agents exit $\tc(s)$ on the same node and at the same round $t <  \Delta_s + T(\del_s) + T(\minn_s)$ if the following two conditions are verified:
\begin{enumerate}
\item Every good agent ends up executing phase $\minn_s$. 
\item $|\mathcal{G}_2| \geq (f+1)(5f+1)+1$.
\end{enumerate}
\end{lemma}

\begin{proof}
Let $\Delta_{\minn_s}=\Delta_s+T(\del_s)$ be the first round in which a good agent starts the execution of phase $\minn_s$. Before proving our lemma, we proceed by proving a series of claims. In the rest of the proof, we assume that the two conditions of the statement are verified. We also assume that every state mentioned in this proof is of phase $\minn_s$. Hence, we omit to precise the phase to which each state belongs.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $\mathcal{A}$ be the set of good agents that start the execution of $\tc(s)$ at round $\Delta_s$.  Note that, $\mathcal{A} \subseteq \mathcal{G}_1$ and by definition $\mathcal{A} \ne \emptyset$.

\noindent \textbf{Claim 1} Let $B$ be an agent of $\mathcal{G}_2$. Agent $B$ executes  $IM(2, 2^s)$ from its initial node. Moreover, for every agent $A$ of $\mathcal{A}$, $B$ records $A$ during its execution of $IM(2, 2^s)$ when $A$ is on its initial node.

\noindent \textbf{Proof of Claim 1}
From Proposition \ref{pro:delayed}, when any good agent starts executing Phase $\minn_s$, it is on its initial node. From the description of Subroutine $\tc(s)$, when executing Phase $\minn_s$, any good agent first {
%$B'$ starts by waiting $r_s=\sum\limits_{j=1}^{s-1}T(\tc(j))+T(EXPLO(2^s))$ rounds in \sta{\szG} before 
performs $IM(2, 2^s)$ which lasts $2T(EXPLO(2^s))$ rounds}. Remember that at the end of $IM(2, 2^s)$, the agent is on its initial node. It then transits to \sta{\swY} in which it remains idle on its initial node for $r_s$ rounds. In view of the definition of set $\mathcal{G}_2$ and Lemma \ref{f:lemma:maxdelay}, we have $2T(EXPLO(2^s)) < {\mathcal{T}(s)} \leq delay_{(A,B)} \leq r_s$. Hence, in view of Corollary \ref{each-phase} and Proposition \ref{pro:delayed}, during the entire execution of $IM(2, 2^s)$ by $B$, $A$ remains on its node in \sta{\swY}. Hence, the claim holds. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\noindent \textbf{Claim 2} Let $A$ be an agent of $\mathcal{A}$ and let $\rho$ be the round in which $A$ transits to \sta{\swY} from \sta{\szH}. At round $\rho$, every agent $B$ of $\mathcal{G}_2$ is in \sta{\szH}. Moreover, agent $A$ (respectively $B$) remains at least {$\mathcal{T}(s)$} rounds in \sta{\swY} (respectively \szH{}) from round $\rho$.  

\noindent \textbf{Proof of Claim 2}
Assume by contradiction that the claim does not hold. In view of the algorithm, $A$ spends exactly $r_s+T(EXPLO(2^s))$ rounds in \sta{\szH} before transiting to \sta{\swY}. By definition of set $\mathcal{G}_2$ and Lemma \ref{f:lemma:maxdelay}, we know that for any agent $B$ of $\mathcal{G}_2$, ${\mathcal{T}(s)} \leq delay_{(A,B)} \leq r_s$. That is, in view of Proposition \ref{pro:delayed} and Corollary \ref{each-phase}, after the first $r_s$ rounds of $A$ in \sta{\szH}, every good agent is also in \sta{\szH}. Moreover, when $A$ transits to \sta{\swY} from \sta{\szH}, for every good agent of $\mathcal{G}_2$, it remains to spend at least {$\mathcal{T}(s)$} rounds in \sta{\szH}. In the same manner, as $A$ waits $r_s > { \mathcal{T}(s)}$ rounds while in \sta{\swY}, the claim holds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\noindent \textbf{Claim 3} If $f \geq n$, there are at least $(5f+2)$ agents that share the same node initially. 
  
 
\noindent \textbf{Claim 3} Assume that $f <n$.  Let $\rho$ be the round in which an agent $A$ of $\mathcal{A}$ transits to \sta{\swY} from \sta{\szH}. At least $(5f+2)$ good agents meet at some round $\rho \leq \rho ' < {\rho+ \mathcal{T}(s)}$.   

\noindent \textbf{Proof of Claim 3} % Observe that if $f \geq n$, by the pigeonhole principle, there are at least $(5f+2)$ agents that are on the same node initially. Hence, the claim holds.
The proof of Claim 3 requires three steps. We first show that there exists a round $\rho \leq x < \rho+\mathcal{T}(s){-2T(EXPLO(2^s))}$ from which no agent of $\mathcal{G}_2$ updates its imperfect map during $2T(EXPLO(2^s))$ rounds. Then, we explain that at round $\rho$, every good agent of $\mathcal{G}_1$ is still recorded in the imperfect map of any good agent $B$ of $\mathcal{G}_2$. At last, we prove that this implies that the claim holds.

By Claim 2, from round $\rho$ to round $\rho+{\mathcal{T}(s)}-1$, every agent of $\mathcal{G}_2$ is in \sta{\szH} and every agent of $\mathcal{A}$ is in \sta{\swY}. Since every agent $A$ of $\mathcal{G}_2$ records at most $f < n < 2^s$ Byzantine agents on each node, $A$ performs at most $2^sT(EXPLO(2^s))$ updates of its imperfect map $P$. On another hand, from Lemma \ref{f:lemma:maxdelay} and Proposition \ref{pro:delayed}, we know that for any pair of good agents $A$ and $B$, if $delay_{(A,B)} \geq 0 $, $A$ starts the execution of $IM(2,2^s)$, $delay_{(A,B)}$ rounds before $B$ from its initial node. Since when a good agent $A$ is awakened on its initial node $u$, all the good dormant agents on $u$ are also awakened, all the good agents on $u$ compute the same imperfect map when executing $IM(2, 2^s)$ during phase $\minn_s$. Hence, the agents of $\mathcal{G}_2$ have at most $2^s$ distinct imperfect maps. So, after at most $4(2^sT(EXPLO(2^s)))^2 = \mathcal{T}(s) - 2T(EXPLO(2^s))$ rounds from round {$\rho$}, no agent of $\mathcal{G}_2$ updates its imperfect map.

Now assume by contradiction, that at round $x$, there exists a good agent $A$ of $\mathcal{G}_1$ which is not recorded by some good agent $B$ of $\mathcal{G}_2$ \ie there is no list $L_i$ of the imperfect map $P$ of $B$ containing a couple $(delay(B, A), \ell_A)$ with $\ell_A$ the label of $A$ and $i$ some integer such that after the $i$ first edge traversals of $T(EXPLO(2^i))$ from its initial node $B$ reaches the initial node of $A$. In view of Claim 1, when in \sta{\szG}, $B$ recorded $A$. This means that, before it enters \sta{\szH}, such a couple exists. Hence, at some rounds before $x$, while in \sta{\szH}, $B$ removes these couples from its list. In view of the description of this state, we know that when it performs one of this removals, $B$ is in the initial node of $A$, while the latter is not, and $y - delay(B, A) > r_s + T(EXPLO(2^s))$ with $y$ the number of rounds spent by $B$ in \sta{\szH}. However, by Corollary~\ref{each-phase}, agent $A$ enters \sta{\szH} $|delay(B, A)|$ rounds before agent $B$, and thus enters \sta{\swY} in its initial node when $B$ has spent exactly $r_s + T(EXPLO(2^s)) + delay(B,A)$ rounds in \sta{\szH}. This concludes the second step of this proof.

In view of the description of our algorithm along with Claim 2, we know that the imperfect map of every agent of $\mathcal{G}_2$ remains useful (refer to definition \ref{def:use}) from round $x$ to round $x+2T(EXPLO(2^s))-1$. We say that a given node $u$ is a target node of an agent $A$ of $\mathcal{G}_2$ at round $x$ if $u$ is the node that is reached after performing the first $(j-1)$ edge traversals of $EXPLO(2^s)$ from the initial node of $A$ and $j$ is the bottom index of the imperfect map of $A$ at round $x$. Let $\mathcal{Q}$ be the set of nodes verifying the following condition: $u$ is in $\mathcal{Q}$ if $u$ is the target node of an agent of $\mathcal{G}_2$ at round $x$.

We proceed at showing that among the nodes of $\mathcal{Q}$, at least $|\mathcal{Q}|-1$ of them host a Byzantine agent at round $x+ 2T(EXPLO(2^s))-1$. By assumption, no agent of $\mathcal{G}_2$ updates its imperfect map from round $x$ to round $x+ 2T(EXPLO(2^s))-1$. Moreover, every agent of $\mathcal{G}_2$ spends at most $2T(EXPLO(2^s))-1$ rounds to reach its target node from round $x$. Hence, at round $x+2T(EXPLO(2^s))-1$, every agent $B$ of $\mathcal{G}_2$ is on its target node. It follows that at round $x+ 2T(EXPLO(2^s))-1$, on each node of $\mathcal{Q}$ there is at least one agent $A$ such that $(delay_{(B,A)}, \ell_B)$ is the smallest couple in the imperfect map of an agent $B$ of $\mathcal{G}_2$. If $A$ is a good agent then $A$ is the agent of $\mathcal{A}$ with the smallest label. Since we cannot have two good agents with the same label, we deduce that at least $|\mathcal{Q}|-1$ nodes of $\mathcal{Q}$ host a Byzantine agent at round $x+ 2T(EXPLO(2^s))-1$. 

Thus, $|\mathcal{Q}| \leq f+1$. Since $|\mathcal{G}_2| \geq (5f+1)(f+1)+1$, by the Pigeonhole principle, it follows that at least $5f+2$ agents share the same node at round $x+2T(EXPLO(2^s))-1$, which concludes the proof.

%Observe that we have only considered in our discussion the agents of $\mathcal{A}$ instead of $\mathcal{G}_1$. Indeed, agents of $\mathcal{G}_1-\mathcal{A}$ impact neither the behavior of the agents of $\mathcal{A}$ nor the ones of $\mathcal{G}_2$, they are also not needed to ensure the meeting of at least $(5f+2)$ agents on the same round. As a side node, from round $\rho$ to round $\rho+\mathcal{T}(s)+2T(EXPLO(2^s))$, the agents of $\mathcal{G}_2-\mathcal{A}$ are either in \sta{\swY} on their initial node or in \sta{\szH}. % fixme




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Claim 4} At least $(4f+2)$ good agents start the execution of $\swD ({\mathcal{R}_s+r_s}, 2^s)$ of phase $\minn_s$ on the same node and at the same round.

\noindent \textbf{Proof of Claim 4} Since every good agent executes the same actions while in phase $\minn_s$ before transiting to \sta{\szI}, by Lemma \ref{f:lemma:maxdelay}, Proposition \ref{pro:delayed} and Corollary \ref{each-phase}, every good agent transits to \sta{\szI} of phase $\minn_s$ at most $r_s$ rounds after an agent of $\mathcal{A}$. Let $\alpha$ be the largest number of agents which are either in \sta{\szG}, \swY{} or \szH{} and that met on the same node $u$ at some round $\Delta_{\minn_s}+\beta \leq \Delta_{\minn_s}+ T(\minn_s)$. If there are several such rounds, we consider the one with the largest value of $\beta$. By Claim 3, we know that if $f<n$ then $\alpha \geq (5f+2)$. Note that in the case where $f \geq n$, since {the total number of good agents is at least $2((5f+1)(f+1)+1)$}, by the pigeonhole principle we can also deduce that  $\alpha \geq (5f+2)$. Let $\mathcal{Y}$ be the set of good agents in either \sta{\szG}, \swY{} or \szH{} on node $u$ at round $\Delta_{\minn_s}+\beta$. When a good agent $A$ of $\mathcal{Y}$ transits to \sta{\szI}, it is on its initial node (refer to the description of \sta{\szH}). Moreover, $A$ repeats exactly the same waiting periods and edge traversals executed from the beginning of phase $\minn_s$ to $\Delta_{\minn_i}+ \beta$ in order to rebuild the group of agents that was on node $u$ at round $\Delta_{\minn_s}+\beta$. More precisely, let $t$ and $t'$ be respectively the round in which $A$ starts the execution of phase $\minn_s$ and the round in which $A$ enters \sta{\szI}. Let $i$ the integer such that $t+i= \Delta_{\minn_s}+\beta$. From round $t'$ to round $t'+i-1$, agent $A$ repeats  exactly the same waiting periods and edges traversals: for each integer $y$ in $\{0,1,\ldots,\beta-1\}$, if agent $A$ remains idle (resp. leaves the current node via a port $o$) from round $t+y$ to round $t+y+1$, then agent $A$ remains idle (resp. leaves the current node via port $o$) from round $t'+y$ to $t'+y+1$. At round $t'+i$, agent $A$ is in node $u$  and starts the execution of  $\swD ({\mathcal{R}_s+r_s}, 2^s)$. However,  from the algorithm, every good agent spends the same number of rounds in phase $\minn_s$ before transiting to \sta{\szI}: let us denote this number by $\mathcal{W}$. That is, $t'+i=t+\mathcal{W}+i= \Delta_{\minn_s}+\beta+ \mathcal{W}$. Hence, every agent of $\mathcal{Y}$ is on $u$ and hence starts the execution of  $\swD ({\mathcal{R}_s+r_s}, 2^s)$ at round $\Delta_{\minn_s}+\beta+\mathcal{W}$. Since $|\mathcal{Y}| \geq (5f+2)-f$, the claim holds.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

We can now prove our lemma. From Claim 4, we know that a group of at least $4f+2$ agents start the execution of $\swD ({\mathcal{R}_s+r_s}, 2^s)$ on the same node and at the same round. On another hand, as every good agent spends exactly $\mathcal{R}_i$ rounds executing phase $\minn_s$ before entering \sta{\szI}, by Lemma \ref{f:lemma:maxdelay}, Corollary \ref{each-phase} and Proposition \ref{pro:delayed}, we can deduce that for any good agent $A$, $A$ enters \sta{\szI} between round $\Delta_{\minn_s}+ \mathcal{R}_i-1$ and round $\Delta_{\minn_s}+ \mathcal{R}_i+ r_i-1$. While in \sta{\szI}, every good agent $A$ repeats the same edge traversals and waiting periods executed from the beginning of phase $\minn_s$ to join a node $u$ on which $A$ was with the largest number of agents. That is, for any pair of good agents $A$ and $B$, if without loss of generality $A$ starts the execution of $\swD ({\mathcal{R}_s+r_s}, 2^s)$ before $B$ then $B$ starts the execution of $\swD ({\mathcal{R}_s+r_s}, 2^s)$ at most $\mathcal{R}_s + r_s$ rounds after $A$. Hence, from Theorem \ref{block2:proof:theo}, we can deduce that all the good agents exit $\swD ({\mathcal{R}_s+r_s}, 2^s)$ on the same node and at the same round $t' \leq \Delta_{\minn_s}+ T(\minn_s)$. Remember that $f \geq \mathcal{F}_{\min}=2^{2^{\lfloor\log \log f\rfloor}}$.  As $\mathcal{F}_{max}=(\mathcal{F}_{min})^2$, we have $2((5 \mathcal{F}_{min}+1) (\mathcal{F}_{min}+1)+1) \geq 4\mathcal{F}_{max}+2$. From the description of phase $\minn_s$, when at least $4\mathcal{F}_{max}+2$ good agents exit $\swD ({\mathcal{R}_s+r_s}, 2^s)$ on the same node and the same round, each of them sets its variable $InGroup$ to $true$ and also exit $\tc(s)$ which proves the lemma.

 
 
\end{proof}


Using similar arguments to the ones used to prove Lemma \ref{f:lemma:minn}, we can prove the following lemma.

\begin{lemma}\label{f:lemma:majj}
%A group of at least $4\mathcal{F}_{max}+2$ good agents exit phase $\majj_s$ on the same node and at the same round $t \leq \Delta_s + T(\del_s) + T(\minn_s) + T(\majj_s)$ if the following two conditions are verified:

All the good agents exit phase $\majj_s$ on the same node and at the same round $t \leq \Delta_s + T(\del_s) + T(\minn_s) + T(\majj_s)$ if the following two conditions are verified:

\begin{enumerate}
\item Every good agent ends up executing phase $\majj_s$.

\item $|\mathcal{G}_2| < (5f+1)(f+1)+1$.
\end{enumerate}

\end{lemma}
%
%\begin{proof}
%Let $\Delta_{\majj_s}=\Delta_{\minn_s}+T(\minn_s)$ be the first round in which a good agent starts the execution of phase $\majj_s$.  Let $\mathcal{A}'$ be the set of the latest good agents that execute $\tc(s)$.  Observe that for any pair of agents $A$ of $\mathcal{A}'$ and $B$ of $\mathcal{G}_1$, $delay(B,A) > 2\mathcal{T}(s)$ holds.
%
%Before proving our lemma, we proceed by proving a series of claims. In the rest of the proof, we assume that the two conditions of the statement are verified. We also assume that every state mentioned in this proof is of phase $\majj_s$. That is, we omit to precise the phase to which each state belongs to. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\noindent \textbf{Claim 1} 
%let $A$ be an agent of $\mathcal{G}_1$. Agent $A$ starts the execution of $IM(3, 2^s)$ from its initial node. Moreover, for every agent $B$ of $\mathcal{A}'$, $A$ records $B$ during its execution of $IM(3, 2^s)$ when $B$ is on its initial node. 
%
%
%\noindent \textbf{Proof of Claim 1}
%
%By Corollary \ref{each-phase}, Proposition \ref{pro:delayed} and Lemma \ref{f:lemma:maxdelay},  we know that every good agent starts executing phase $\majj_s$ from its initial node by round $\Delta_{\majj_s}+ r_s-1$. In view of the description of phase $\majj_s$, when a good agent $B'$ starts executing phase $\majj_s$, it first waits $r_s+2T(EXPLO(2^s))+2\mathcal{T}(s)$ rounds on its current node before transiting to \sta{\szH} and executing  $IM(3, 2^s)$ which lasts $2T(EXPLO(2^s))$ rounds. By the definitions of sets $\mathcal{G}_1$ and $\mathcal{A}'$, $delay(A,B) > 2\mathcal{T}(s)$. Since $2T(EXPLO(2^s)) < 2 \mathcal{T}(s)$, we can deduce that during the entire execution of $IM(3, 2^s)$ by $A$, $B$ is on its current node in \sta{\swY}. Thus, the claim holds. 
%
%
%\noindent \textbf{Claim 2} 
%Let $A$ be the last agent of $\mathcal{G}_1$ to execute phase $\majj_s$ and let $\rho$ be the round in which $A$ enters \sta{\szH}. At round $\rho$, every agent $B$ of $\mathcal{A}'$ is in \sta{\swY} while every agent $A'$ of $\mathcal{G}_1$ is in \sta{\szH}. Moreover, agent $A'$ (respectively agent $B$) remains at least $2 \mathcal{T}(s)$ rounds in \sta{\szH}  (respectively \sta{\swY}) from round $\rho$.
%
%
%\noindent \textbf{Proof of Claim 2} 
%Assume by contradiction that the claim does not hold. In view of the description of phase $\majj_s$, any good agent $B'$ which starts executing phase $\majj_s$ starts by waiting $r_s+ 2T(EXPLO(2^s))+2\mathcal{T}(s)$ rounds on its current node while in \sta{\swY} before transiting to \sta{\szH} and performing $IM(3, 2^s)$  which lasts $2T(EXPLO(2^s))$ rounds. At the end of $IM(3,2^s)$, $B'$ executes \sth{Search} that lasts at least $r_s$ rounds and at most $r_s+T(EXPLO(2^s))-1$ rounds. It then waits $r_i+T(EXPLO(2^s))-x$ rounds before transiting to \sta{\szI} where $x$ is the number of rounds agent $A$ spent executing \sth{Search}. Since, by definition, for any pair of agents $X$ of $\mathcal{G}_1$ and $Y$ of $\mathcal{A}'$, $delay_{(X,Y)} > 2 \mathcal{T}(s)$ holds, when agent $A$ enters \sta{\szH} at round $\rho$, every agent of $\mathcal{A}'$ remains in \sta{\swY} for at least $2\mathcal{T}(s)$ rounds from $\rho$. Hence, the claim holds. 
%
%
%\noindent \textbf{Claim 3} Assume that $f <n$. Let $\rho$ be the round in which the last agent of $\mathcal{G}_1$ enters \sta{\szH}. At least $(5f+2)$ good agents meet at some round $\rho + 2T(EXPLO(2^s))-1 \leq \rho' \leq \rho+  2T(EXPLO(2^s))+ \mathcal{T}(s)$.
%
%\noindent \textbf{Proof of Claim 3} 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% To prove Claim 3, we first show that if there exists a round $\rho + 2T(EXPLO(2^s)) -1 \leq x < \rho+  \mathcal{T}(s)-1$ from which no agent of $\mathcal{G}_1$ updates its imperfect map during $2T(EXPLO(2^s))$ rounds then the claim holds. Observe that since every good agent executes phase $\majj_s$, by lemma \ref{f:lemma:del}, $\mathcal{A}' \ne \emptyset$ and by claim 2, the imperfect map of every agent of $\mathcal{G}_2$ remains useful (refer to definition \ref{def:use}) from round $x$ to round $x+2T(EXPLO(2^s))-1$. Let  $\rho + 2 T(EXPLO(2^s))-1 \leq x < \rho+\mathcal{T}(s)-1$ be a round from which no agent of $\mathcal{G}_1$ updates its imperfect map for at least $2T(EXPLO(2^s))$ rounds. We say that a given node $u$ is a target node of an agent $A$ of $\mathcal{G}_1$ at round $x$ if $u$ is the node that is reached after performing the first $(j-1)$ edge traversals of $EXPLO(2^s)$ from the initial node of $A$ and $j$ is the up index of the imperfect map of $A$ at round $x$. Let $\mathcal{Q}$ be the set of nodes verifying the following condition: $u$ is in $\mathcal{Q}$ if $u$ is the target node of an agent of $\mathcal{G}_1$ at round $x$.
%
%We proceed at showing that among the nodes of $\mathcal{Q}$, at least $|\mathcal{Q}|-1$ of them host a Byzantine agent at round $\rho+ 2T(EXPLO(2^s))-1$. Since by assumption, no agent of $\mathcal{G}_1$ updates its imperfect map from round $x$ to round $x+ 2T(EXPLO(2^s))-1$, it follows that on each node of $\mathcal{Q}$ there is at least one agent $B$ such that $(delay_{(A,B)}, \ell_B)$ is the largest couple in the imperfect map of an agent of $\mathcal{G}_1$. By definition such an agent $B$ and claim $1$, if $B$ is a good agent then $B$ is the agent of $\mathcal{A}'$ with the largest label.   As every agent of $\mathcal{G}_1$ spends at most $2T(EXPLO(2^s))-1$ rounds to reach its target node after round $x$, at round $x+2T(EXPLO(2^s))-1$, every agent $A$ of $\mathcal{G}_1$ is on its target node. We can deduce hence deduce that $|\mathcal{Q}|-1$ nodes of $\mathcal{Q}$ host a Byzantine agent at round $x+2T(EXPLO(2^s))-1$. That is $|\mathcal{Q}| \leq f+1$. On another hand, since $|\mathcal{G}_1| \geq (5f+1)(f+1)+1$, by the Pigeonhole principle, it follows that at least $5f+2$ agents share the same node at round $x+2T(EXPLO(2^s))-1$.  
%
%%Observe that we have only considered in our discussion the agents of $\mathcal{A}'$ instead of $\mathcal{G}_2$. This is due to that fact that these agents impact neither the behavior of the agents of $\mathcal{A}'$ (that remain in \sta{\swY} on their initial node) nor the ones of $\mathcal{G}_1$ and they are not needed to ensure the meeting of at least $(5f+2)$ agents on the same round. Observe that from round $x$ to round $x+2T(EXPLO(2^s))$, the agents in $\mathcal{G}_2-\mathcal{A}'$ are either in \sta{\swY} on their initial node or in \sta{\szH} of phase $\majj_s$.  
%
%If round  {$x$} exists, then the claim holds. So to conclude the proof of this claim, it remains to show the existence of round {$x$}. By claim 2, from round $\rho$ to round $\rho+2\mathcal{T}(s)$, every agent of $\mathcal{G}_1$ are in \sta{\szH} while every agent of $\mathcal{A}'$ is in \sta{\swY}. Since every agent $A$ of $\mathcal{G}_1$ records at most $2^s$ Byzantine agents that pretend to be of $\mathcal{G}_2$ on each node while executing $IM(3, 2^s)$ that lats $2T(EXPLO(2^s))$ rounds, $A$ performs at most $T(EXPLO(2^s)). 2^s$ updates of its imperfect map $P$. 
%
% On another hand, from Lemma \ref{f:lemma:maxdelay} and Proposition \ref{pro:delayed}, we know that for any pair of good agents $A$ and $B$, if $delay_{(A,B)} \geq 0 $, $A$ starts the execution of $IM(3,2^s)$ from its initial node, $delay_{(A,B)}$ rounds after $B$. Since when a good agent $A$ is awakened on its initial node $u$, all the good dormant agents on $u$ are also awakened, all the good agents on $u$ compute the same imperfect map when executing $IM(2, 2^s)$ during phase $\minn_s$. Hence, there are at most $2^s$ distinct imperfect maps of the agents of $\mathcal{G}_2$. So, after at most $\mathcal{T}(s)- 2T(EXPLO(2^s))=4(2^s T(EXPLO(2^s))^2$ rounds from round {$\rho$}, no agent of $\mathcal{G}_1$ updates its imperfect map. This proves the existence of round {$x$} and hence the claim.
%
%\noindent \textbf{Claim 4}
%
%At least $(4f+2)$ agents start the execution of $\swD(2\mathcal{R'}_s, 2^s)$ of phase $\majj_s$ on the same node and at the same round.  
%
%\noindent \textbf{Proof of Claim 4}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%As every good agent executes the same actions while in phase $\majj_s$ before transiting to \sta{\szI}, by Lemma \ref{f:lemma:maxdelay}, Proposition \ref{pro:delayed} and Corollary \ref{each-phase}, when an agent of $\mathcal{A}$ enters \sta{\szI}, every good agent also transits to \sta{\szI}, $r_s$ rounds later at the latest. Let $\alpha$ be the largest number of agents which are either in \sta{\swY} or \szH{} and that met on the same node $u$ at some round $\Delta_{\majj_s}+\beta \leq \Delta_{\minn_s}+ T(\majj_s)$ (during their execution of phase $\majj_s$). If there are several such rounds, we consider the one with the largest value of $\beta$. By claim 3, we know that if $f<n$, $\alpha \geq (5f+2)$ holds. Observe that in the case where $f \geq n$, since the total number of good agents is at least $2((5f+1)(f+1)+1)$, by the pigeonhole principle, we can also deduce that $\alpha \geq (5f+2)$. Let $\mathcal{Y}$ be the set of good agents on either \sta{\swY} or \szH{} on node $u$ at round $\Delta_{\majj_s}+\beta$. When a good agent $A$ of $\mathcal{Y}$ transits to \sta{\szI}, it is on its initial node (refer to the description of \sta{\szH}). Moreover, $A$ repeats exactly the same waiting periods and edge traversals executed from the beginning of phase $\majj_s$ to $\Delta_{\majj_i}+ \beta$ in order to rebuild the group of agents that was on node $u$ at round $\Delta_{\majj_s}+\beta$. More precisely, let $t$ and $t'$ be respectively the round in which $A$ starts the execution of phase $\majj_s$ and the round in which $A$ enters \sta{\szI}. Let $i$ the integer such that $t+i= \Delta_{\majj_s}+\beta$. From round $t'$ to round $t'+i-1$, agent $A$ repeats  exactly the same waiting periods and edges traversals: for each integer $y$ in $\{0,1,\ldots,\beta-1\}$, if agent $A$ remains idle (resp. leaves the current node via a port $o$) from round $t+y$ to round $t+y+1$, then agent $A$ remains idle (resp. leaves the current node via port $o$) from round $t'+y$ to $t'+y+1$. At round $t'+i$, agent $A$ is in node $u$  and starts the execution of  $\swD (2\mathcal{R}_s, 2^s)$. However,  from the algorithm, every good agent spends the same number of rounds in phase $\majj_s$ before transiting to \sta{\szI}: let us denote this number by $\mathcal{W}$. That is, $t'+i=t+\mathcal{W}+i= \Delta_{\majj_s}+\beta+ \mathcal{W}$. Hence, every agent of $\mathcal{Y}$ is on $u$ and hence starts the execution of  $\swD (2\mathcal{R}_s, 2^s)$ at round $\Delta_{\majj_s}+\beta+\mathcal{W}$. Since $|\mathcal{Y}| \geq (5f+2)-f$, the claim holds.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
% 
%
%We can now prove our lemma. From Claim 4, a group of at least $4f+2$ good agents start the execution of $\swD (2\mathcal{R}_s, 2^s)$ on the same node and at the same round. On another hand, as every good agent spends exactly $\mathcal{R}'_i$ rounds executing phase $\majj_s$ before entering \sta{\szI}, by Lemma \ref{f:lemma:maxdelay}, Corollary \ref{each-phase} and Proposition \ref{pro:delayed}, we can deduce that for any good agent $A$, $A$ enters \sta{\szI} between round $\Delta_{\majj_s}+ \mathcal{R}'_i-1$ and round $\Delta_{\majj_s}+ \mathcal{R}'_i+ r_i-1$. While in \sta{\szI}, every good agent $A$ repeats the same edge traversals and waiting periods executed from the beginning of phase $\majj_s$ to join a node $u$ on which $A$ was with the largest number of agents. That is, for any pair of good agents $A$ and $B$, if without loss of generality $A$ starts the execution of $\swD (2\mathcal{R}'_s, 2^s)$ before $B$ then $B$ starts the execution of $\swD (2\mathcal{R}'_s, 2^s)$ after at most $2\mathcal{R}'_i$ rounds after $A$. Hence, from Theorem \ref{xx} of section \ref{sec:block}, we can deduce that all the good agents exit $\swD (2\mathcal{R}'_s, 2^s)$ on the same node and at the same round $t' \leq \Delta_{\majj_s}+ T(\majj_s)$. Recall $f \geq \mathcal{F}_{\min}=2^{2^{\lfloor\log \log f\rfloor}}$.  As $\mathcal{F}_{max}=(\mathcal{F}_{min})^2$, we have $2((5 \mathcal{F}_{min}+1) (\mathcal{F}_{min}+1)+1) \geq 4\mathcal{F}_{max}+2$. From the description of phase $\majj_s$, when at least $4\mathcal{F}_{max}+2$ good agents exit $\swD (2\mathcal{R}'_s, 2^s)$ on the same node and the same round, each of them sets its variable $InGroup$ to $true$ and also exit $\tc(s)$ which proves the lemma.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
%
%
%
%\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{lemma}
%A group of at least $4\mathcal{F}_{max}+2$ agents starts executing $\sd$, $\sum\limits_{j=1}^{s} \tc(j)$ rounds after $\Delta$ at the latest. 
%\end{lemma}


\begin{lemma}\label{f:lemma:group}
There exists $1 \leq i \leq s$ such that a group of at least {$4\mathcal{F}_{max}+2$} good agents exit their execution of $\tc(i)$ with their respective $InGroup$ variable set to $true$ on the same node and at the same round $t \leq \Delta + \sum \limits_{j=1}^{s}T(\tc(j))$.
\end{lemma}

\begin{proof}
%Assume by contradiction that the lemma does not hold. That is, for all $0 < i \leq s$, every agent exits $tc(i)$ with $InGroup=false$.
Remember that {the total number of good agents is larger than $5\mathcal{F}_{\max}+2$}. Assume that for all $i$ such that $1 \leq i \leq s-1$, no group of at least {$4\mathcal{F}_{\max}+2$} good agents exit their execution of $\tc(i)$ with their respective  $InGroup$ variable set to $true$ on the same node and at the same round $t \leq \Delta + \sum \limits_{j=1}^{i}T(\tc(j))$. From the description of our algorithm, there is at least one good agent $A$ that starts the execution of $\tc(s)$. Let $\Delta_s$ be the first round in which a good agent starts the execution of $\tc(s)$. By Lemma \ref{f:lemma:awake}, every good agent is awake at round $\Delta_s+T(EXPLO(2^s))$. From the description of our algorithm, Lemma \ref{f:lemma:maxdelay} and Corollary \ref{onlyf:timetc},  we know that every good agent starts executing $\tc(s)$ by round $\Delta_s+ r_s-1$. By lemma \ref{f:lemma:del}, we know that if every good agent starts executing $\tc(s)$ by round {$\Delta_s+2\mathcal{T}(s)-1$} then a group of at least {$5\mathcal{F}_{\max}+2$} good agents exit their execution of $\tc(s)$ with their respective  $InGroup$ variable set to $true$ on the same node and at the same round $t \leq \Delta + \sum \limits_{j=1}^{s-1}T(\tc(j))+T(\del_s) < \Delta + \sum \limits_{j=1}^{s}T(\tc(j))$. Hence, we can deduce that there exists a pair of good agents $A$ and $B$ such that $delay_{(A,B)} > {2\mathcal{T}(s)}$. This implies that the set of {all the good agents} can be partitioned into two subsets $\mathcal{G}_1$ and $\mathcal{G}_2$ as defined previously. If $\mathcal{G}_2 \geq (5f+1)(f+1)+1$, by Lemma \ref{f:lemma:minn}, a group of at least {$5\mathcal{F}_{\max}+2$} good agents exit their execution of $\tc(s)$ with their respective  $InGroup$ variable set to $true$ on the same node and at the same round $t \leq \Delta + \sum \limits_{j=1}^{s-1}T(\tc(j))+T(\del_s)+ T(\minn_s) < \Delta + \sum \limits_{j=1}^{s}T(\tc(j))$. Hence, we can deduce that $\mathcal{G}_2 < (5f+1)(f+1)+1$. By Lemma \ref{f:lemma:majj}, in this case too a group of {$5\mathcal{F}_{\max}+2$} good agents exit their execution of $\tc(s)$ with their respective  $InGroup$ variable set to $true$ on the same node and at the same round $t \leq \Delta + \sum \limits_{j=1}^{s}T(\tc(j))$. This concludes the proof of this lemma.

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Let $\mathcal{Y}$ and $\rho$ be respectively the first group of at least $3\mathcal{F}_{max}+2$ good agents that executes $\sd$ and the round in which the agents of $\mathcal{Y}$ exit \sth{\sd}. Note that by lemma \ref{f:lemma:group}, $\mathcal{Y}$ and $\rho$ exist.

{Let $\mathcal{Y}$, $\mathcal{D}_1$ and $\rho$ be respectively the first group of at least {$4\mathcal{F}_{max}+2$} good agents that exit subroutine $\Syn$, the parameter of $\Syn$ executed by the good agents of $\mathcal{Y}$ and the the round in which the agents of $\mathcal{Y}$ exit \sth{\sd}. Let $i$ be a positive integer such that {$4\mathcal{F}_{\max}+2$} good agents of $\mathcal{Y}$ starts the execution of $\sd$ after exiting $\tc(i)$. Note that by lemma \ref{f:lemma:group}, $\mathcal{Y}$, $\rho$ and $i$ exist.} 


\begin{lemma}\label{f:everyoneGroup}
At round {$\rho + \mathcal{D}_1$}, every good agent is in a group of at least {$4\mathcal{F}_{max}+2$} good agents executing {subroutine $\Syn$} and having the same indicator. 
\end{lemma}

\begin{proof}
From the description of our algorithm, we know that all the good agents in $\mathcal{Y}$ are in \sta{\szJ} sharing the same indicator $(t,n)$ at each round from round $\rho+1$ to round $\rho + {\mathcal{D}_1}$.

{We denote by $\mathcal{Z}$ the first group of at least {$4\mathcal{F}_{\max}+2$} good agents to exit $\tc(j)$ for any positive integer $j$. In view of the definition of group $\mathcal{Y}$, we know that $i \leq j$ and hence by Lemma \ref{f:lemma:group}, we can conclude that $i \leq s$.} Note that as soon as a good agent terminates to execute $\tc(\lceil \log n\rceil)$, it remains no dormant good agent. Hence, in view of the algorithm and Property \ref{pro:delayed}, we know that in every round we cannot have two good agents executing $\tc$ with parameters whose positive difference is greater than $\lceil \log n\rceil+1$. That is, at round $\rho-T(\sd)+1$ (i.e., in the last round when the good agents of $\mathcal{Y}$ execute $\tc(i)$), we know that no good agent has started to execute $\tc(i+\lceil \log n\rceil+2)$. We also know that at round $\rho$ every good agent is awake (due to the properties of $\sd$) and no good agent has started to execute $\tc(i+\lceil \log n\rceil+3)$. 

From round $\rho+1$ on, the good agents of $\mathcal{Y}$ start waiting ${\mathcal{D}_1}$ rounds. This is equal to $T(\sd(n))+\sum\limits_{k=1}^{\lceil \log n\rceil+i+3}\tc(k)$ rounds. Thus, if a good agent $B$ ends up executing $\tc(i+\lceil \log n\rceil+3)$, it is in a group of at least {$4\mathcal{F}_{max}+2$} good agents executing {subroutine $\Syn$} and having the same indicator by round $\rho+\sum\limits_{j=1}^{\lceil \log n\rceil+i+2}\tc(j)+2T(EXPLO(2^{i+\lceil \log n\rceil+3}))$ rounds (i.e., by the time it finishes to execute the execution of $EXPLO(2^{i+\lceil \log n\rceil+3})$ and its backtrack in the beginning of $\tc(i+\lceil \log n\rceil+3)$). Otherwise, according to the algorithm, agent $B$ is in a node containing at least {$5\mathcal{F}_{\max}+2$} agents by round $\rho+\sum\limits_{j=1}^{\lceil \log n\rceil+i+2}\tc(j)$, and thus in a group of at least {$4\mathcal{F}_{max}+2$} good agents executing {subroutine $\Syn$} and having the same indicator by round $\rho+\sum\limits_{j=1}^{\lceil \log n\rceil+i+2}\tc(j)+T(\sd)$ (as $f\leq\mathcal{F}_{max}$). Hence, in all cases the lemma holds. 
\end{proof}

%\begin{lemma}\label{f:everyoneGroup}
% At round $\rho + \mathcal{D} - T(\sd)$, every good agent is in a group of at least $3\mathcal{F}_{max}+2$ good agents executing $\Syn(\mathcal{D})$ and having the same indicator. 
% 
%\end{lemma}
%
%\begin{proof}
%%Let assume by contradiction that the lemma does not hold. That is, there exists at least one good agent $B$ such that $B$ is not in a group of at least $3\mathcal{F}_{max}+2$ agents having the same indicator at round $\rho + \mathcal{D}-T(\sd)$. 
%
%From the description of our algorithm, we know that all the good agents in $\mathcal{Y}$ are in \sta{\szJ} sharing the same indicator $(t,n)$ at each round from round $\rho$ to round $\rho + \mathcal{D} - T(\sd)$. Let $i$ be a positive integer such that $\mathcal{Y}$ was created while executing $\tc(i)$ and let $\rho'$ be the round in which all the good agents of $\mathcal{Y}$ exit $\tc(i)$. From Lemma \ref{f:lemma:group}, we know that $i \leq s$. Let $B$ be a good agent which is not in a group of at least $3\mathcal{F}_{\max}+2$ in \sta{\szJ} at round $\rho+1$. 
%
%Let $j$ be the smallest positive integer such that $n \geq 2^j$. We first show that if a good agent is executing $\tc(k)$ for some positive integer $k$ then for every good agent which is executing $\tc(k')$ for some positive integer $k'>k$, we have $k' \leq k+j+1$.  Assume by contradiction that the previous statement is false. That is, there exists a good agent $A$ which is executing $\tc(k')$ with $k' > k+j+1$. Let $C$ be the first agent to execute $\tc(k')$. From the algorithm, we know that $C$ has executed every phase of $\tc(j)$ before hand. Since $n \geq 2^j$, $C$ has visited every node of the graph during its execution of $EXPLO(2^j)$ at the beginning of phase $\del_j$. That is, at round $\Delta_j+ T(EXPLO(2^j))$, every good agent is awake. In view of Property \ref{pro:delayed}, we know that when $C$ executes $\tc(k')$, every good agent which is executing  $\tc(k'')$ for some positive integer $k''$, we have $k'' \geq k'-j$ which is a contradiction.   
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ù%%%%%%%%%%%%%%%%%%%%%%
%
%From the algorithm, $\mathcal{D}=T(\sd(n))+\sum\limits_{j=1}^{\lceil \log n\rceil+i+3}\tc(j)$. Observe that $\mathcal{D} \geq T(\sd(n))+\sum\limits_{w=1}^{j+i+3}\tc(w)$. We next show that every good agent spends at most $\sum\limits_{w=1}^{j+ i+3}\tc(w)$ rounds to join a group of at least $3\mathcal{F}_{max}+2$ good agents executing $\Syn(\mathcal{D})$ and having the same indicator. In view of the properties of $\sd$, we know that $B$ is awake at round $\rho$. We discuss the following two cases: 
%
%\begin{enumerate}
%\item Agent $B$ is not awake at round $\rho'$. In this case, $B$ spends at most $\sum\limits_{j=1}^{ j}\tc(j)$ rounds after $\rho$ to be sure to join a group of at least $3\mathcal{F}_{\max}+2$ good agents in \sta{\szJ} with the same indicator. 
%
%\item Agent $B$ is awake at round $\rho'$. We have shown that at round $\rho'$, $B$ is executing $\tc(k)$ with $k \leq i+j+1$. Let us first assume that $2^k <n$. Agent $B$ spends at most $\sum\limits_{w=1}^{j}\tc(w)$ rounds to finish the execution of $\tc(j)$ after $\rho'$. Let $\gamma$ be the round in which $B$ finishes the execution of $\tc(j)$. In view of the algorithm, since agent $B$ spends exactly  $2T(EXPLO(2^{j}))+ 2T(\swD(4\mathcal{T}(j), 2^{j}, 2^{j})) + T(\sd(2^{j}))$ rounds executing phase $\del_{j}$. At round $\gamma$, we know that all the agents of $\mathcal{Y}$ finished the execution of $\sd$. On another hand, as $\sum\limits_{w=1}^{j}\tc(w) < \mathcal{D}$, at round $\gamma$ all the good agents of $\mathcal{Y}$ are in \sta{\szJ} sharing the same indicator. Moreover, all good agents of $\mathcal{Y}$ remain in \sta{\szJ} sharing  the same indicator for at least $T(\tc(j+1))+T(\tc(j+2))$ rounds from round $\gamma$. Agent $B$ then spends at most $T(EXPLO(2^{j+1}))$ rounds from round $\gamma$, to join $\mathcal{Y}$ if it did not meet a group of at least $3\mathcal{F}_{\max}+2$ agents in \sta{\szJ} sharing the same indicator before hand. 
%
%Let us now assume that $2^k  \geq n$. As $k \leq i+j+1$, $B$ spends at most $T(\tc(k))+T(\tc(k+1))$ rounds to be sure that the agents of $\mathcal{Y}$ have finished the execution of $\sd$. As $T(\tc(k))+T(\tc(k+1)) < \mathcal{D}$, when $B$ performs $EXPLO(2^{k+2})$, it is sure to join $\mathcal{Y}$ if it did not meet a group of at least $3\mathcal{F}_{\max}+2$ agents in \sta{\szJ} sharing the same indicator before hand.  
%
%
%\end{enumerate}
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%As $\mathcal{Y}$ was created during the execution of $\tc(i)$ for some positive integer $i$. We know that $B$ is executing $\tc(m)$ such that $m \leq i+j+1$. When the good agents of $\mathcal{Y}$ exit $\sd$, they know the value $n$ and hence they compute the value $s'=i+j+1$. As the agents in $\mathcal{Y}$ waits $\mathcal{D}=T(\sd(n))+ \sum\limits_{w=1}^{s'+3}$.
%
%
%
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%We start by showing that when all good agents of $\mathcal{Y}$ exit $\tc(i)$, $B$ is either asleep or executing $\tc(j)$ for a positive integer $j \leq s$. Assume by contradiction that $B$ is neither asleep nor executing $\tc(j)$ for a positive integer $j \leq s$. That is $B$ is either awake and executing $\tc(j)$ with $j>s$ or it is awake but it is not executing $\tc(j)$ for a some positive integer $j$. From the algorithm, if $B$ is awake and not executing subroutine $\tc(j)$ for a some positive integer $j$ then $B$ is part of a group of at least $3\mathcal{F}_{\max}+2$ good agents. Let us refer to this group by $\mathcal{Y}'$. After exactly $T(\sd(n))$ from $\rho'$, that is at round $\rho$, all good agents in $\mathcal{Y}'$ are in \sta{\szJ} which is a contradiction. 
%%
%%Assume now that $B$ is executing $\tc(j)$ with $j>s$. Let $C$ be the first good agent to execute $\tc(j)$. From the algorithm, we know that $C$ has executed $\tc(s)$ before hand. Moreover, from Proposition \ref{pro:delayed}, $C$ is also the first one to execute $\tc(s)$. Let us consider the system during the execution of $\tc(s)$ by $C$. From Lemma \ref{f:lemma:awake}, we know that when $C$ finishes the execution of the first $T(EXPLO(2^s))$ during phase $\del_s$, every good agent is awake. Observe that, by assumption, no group of at least $4\mathcal{F}_{\max}+2$ agents exit $\tc(k)$ for any positive integer $k$ from round $\Delta_s$ to round $\Delta_s+ T(\tc(s))-1$ (since $\mathcal{Y}$ is the first group to do so). Hence, in view of Lemma \ref{f:lemma:del}, we know that there exists a pair of agents $A$ and $A'$ such that $delay_{(A,A')} > 4\mathcal{T}(s)$. When $C$ starts the execution of phase $\minn_s$, $C$ starts by waiting $r_s= \sum\limits_{j=1}^{s-1}\tc(j)+ T(EXPLO(2^s))$ rounds in \sta{\szG} before executing $IM(2,2^s)$. As every agent is awake when $C$ starts the execution of $\minn_s$ and since no group exit $\tc(k)$ for some positive integer $k$ before round $\Delta_s+T(\tc(s))-1$, in view of  Lemma \ref{f:lemma:minn}, we know that $|\mathcal{G}_2| < (f+1)(5f+1)+1$. Nevertheless, when $B$ starts the execution of phase $\majj_s$ it also starts by waiting at least $r_s= \sum\limits_{j=1}^{s-1}\tc(j)+ T(EXPLO(2^s))$ rounds in \sta{\swY} and in the same manner, since no group of at least $4\mathcal{F}_{\max}+2$ agents exit $\tc(k)$ for any positive $k$ before round $\Delta_s+ T(\tc(s))$, every good agent ends up executing phase $\majj_s$. By Lemma \ref{f:lemma:majj}, we know that in this case all the good agents exit $\tc(s)$ on the same node and at the round. That is, $C$ does not execute $\tc(k')$ for any positive integer $k'>s$. This implies that agent $B$ does not exist which is a contradiction. 
%
%
%
%%If $B$ exists then by Lemmas \ref{f:lemma:del}, \ref{f:lemma:minn} and \ref{f:lemma:majj}, $i <s$. As $B$ is awake at round $\rho$, if $B$ is already executing $\tc(s)$ then after at most $T(\tc(s))$ rounds, $B$ performs $EXPLO(2^{s+1})$. As $\tc(s)+T(EXPLO(2^{s+1}) \leq \sum\limits_{j=1}^{\lceil \log n\rceil}\tc(j)$, $B$ is sure to meet $\mathcal{Y}$ while all the good agents of $\mathcal{Y}$ are still in \sta{\szJ} sharing the same indicator $(t,n)$ if it did not meet another group of at least $3\mathcal{F}_{\max}+2$ good agents in \sta{\szJ} sharing the same indicator $(t',n)$. By contrast, in the case where $B$ is not executing $\tc(s)$it spends at most $\sum\limits_{j=1}^{s-1} \tc(j)$ rounds from $\rho$ to starts the execution of $\tc(s)$ and then it spends $T(EXPLO(2^s))$ rounds to visit every node of the graph. As $\sum\limits_{j=1}^{s-1} \tc(j)+T(EXPLO(2^s)) < \sum\limits_{j=1}^{\lceil \log n\rceil}\tc(j)$, if $B$ does not meet a prior group of at least $3\mathcal{F}_{\max}+2$ agents in \sta{\szJ} with the same indicator $(t',n)$, it does meet $\mathcal{Y}$ while all the good agent of $\mathcal{Y}$ are still in \sta{\szJ} with the same indicator $(t,n)$. 
%
%
%From the discussion above, we can deduce that the lemma holds.
%
%
%   
%
%
%
%%From the description of our algorithm, we know that if a group $\mathcal{X}$ of at least $4\mathcal{F}_{\max}+2$ agents exit $\tc(i)$ for some positive integer $i$
%%then $\mathcal{X}$ contains at least $3\mathcal{F}_{\max}+2$ good agents. Moreover, all good agents of $\mathcal{Y}$, are in \sta{\szJ}, having the same indicator $(t,n)$ at each round from round $\rho$ to round $\rho+ \mathcal{D}- T(\sd)$. At round $\rho$, every good agent is awake (recall that during the execution of $\sd$, every node of the graph is visited by at least one good agent). That is, agent $B$ wakes-up at round $\rho$ at the latest. When agent $B$ wakes-up, it starts executing $\tc(1)$ and then spends at most $\sum\limits_{j=1}^{s-1}\tc(j)+ 2T(EXPLO(2^s))$ rounds to enter \sta{\szJ} either after executing line \ref{setVariable} of algorithm \ref{onlyf:algo:main} or after meeting with a group of at least $3\mathcal{F}_{max}+2$ agents sharing the same indicator $(t,n)$ with $t < \mathcal{D}$. Hence, at round $\rho+\sum\limits_{j=1}^{s-1}\tc(j)+ 2T(EXPLO(2^s))$ every good agent is in a group of least $3\mathcal{F}_{max}+2$ agents having the same indicator which proves the lemma.
%\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{Let $\mathcal{W}$ be the set of every group of at least {$4\mathcal{F}_{\max}+2$} good agents that starts executing subroutine $\Syn$ from the same node and from the same round and let $\mathcal{W}_{\mathcal{D}}$ be a set of integers such that $x$ is in $\mathcal{W}_{\mathcal{D}}$ iff there exits a group $\Lambda$ of $\mathcal{W}$ which executes at some point $\Syn(x)$. We set $d= \max \{\mathcal{D}$, $\mathcal{D} \in \mathcal{W}_{\mathcal{D}}\}$.}
 
\begin{lemma}\label{lemma:cmp}
Every good agent discovers $d$ while executing $\cmp(n)$. 
\end{lemma}


\begin{proof}

%Let $\mathcal{W}$ be the set of every group of at least $3\mathcal{F}_{\max}+2$ good agents that starts executing {Subroutine $\Syn$} from the same node and from the same round. %Since every group of $\mathcal{W}$ spends exactly $\mathcal{D}$ rounds executing $\Syn(\mathcal{D})$, 
{In view of the definition of $d$, by Lemma \ref{f:everyoneGroup}, we know that every group of $\mathcal{W}$ starts the execution of $\cmp(n)$ by round $\rho + \mathcal{D}_1+ d$}.

%From the description of the algorithm and  Lemma \ref{f:everyoneGroup}, we know that every good agent ends up executing $\cmp(n)$.


%From the description of subroutine $\cmp(n)$, we know that a good agent $A$ updates its variable $\mathcal{D}'$ only when it meets a group of at least $\mathcal{F}_{\max}+1$ agents all in a same predefined set of states while executing either $\Syn(\mathcal{D})$ or $\cmp(n)$ or $\swD(\mathcal{D}',n)$. In view of the algorithm, we know that no group of Byzantine agents can mimic such a group.

Let $y$ be the group of at least $\mathcal{F}_{\max}+1$ good agents of $\mathcal{Y}$ that perform $EXPLO(n)$ during their execution of $\cmp(n)$. By the algorithm, for every group $\Lambda$ of $\mathcal{W}$ that starts executing {subroutine $\Syn(\mathcal{J})$} from round $x$ on node $u$, we know that from round $x$ to round $x+{\mathcal{J}}+2T(EXPLO(n))+1$, at least $\mathcal{F}_{\max}+1$ good agents of $\Lambda$ are idle on $u$. More precisely, from round $x$ to round $x+{\mathcal{J}}-1$, all the good agents of $\Lambda$ are in \sta{\szJ} sharing the same indicator while from round $x+{\mathcal{J}}$ to round $x+{\mathcal{J}}+2T(EXPLO(n))+1$, there are at least $\mathcal{F}_{\max}+1$ good agents of $\Lambda$ on $u$ in either \sta{\szK} or \szL{}. Hence, using Lemma \ref{f:everyoneGroup}, we know that all the good agents of $y$ meet at least $\mathcal{F}_{\max}+1$ good agents of each group of $\mathcal{W}$. That is, when the good agents of $y$ finish the backtrack of the last $EXPLO(n)$ performed, all the good agents of $y$ assigns to $\mathcal{D}'$ the value of $d$. Also, from the description of $\cmp(n)$, all the good agents of $\mathcal{Y}$ exit $\cmp(n)$ with $\mathcal{D}'=d$.

%On another hand, observe that the node $u$ on which the good agents of $y$ start the execution of $\swD(d,n)$ is the same node as the one from which all the good agents of $\mathcal{Y}$ started their execution of $\Syn(\mathcal{d})$. That is, from the description of $\swD(d,n)$, we know that all the good agents of $\mathcal{Y}$ remain idle during at least $d$ rounds from the beginning of their execution of $\swD(d,n)$ on $u$. 


It remains to show that all the good agents of any other group of $\mathcal{W}- \{\mathcal{Y}\}$ also discover $d$. Assume by contradiction that there is a round $t$ and a group $\Gamma$ of $\mathcal{W}- \{\mathcal{Y}\}$ such that the good agents of $\Gamma$ finishes the execution of $\cmp(n)$ at round $t$ but one of its good agents has its variable $\mathcal{D}'\ne d$. Without loss of generality, we assume that $t$ is the first round for which such a situation occurs.

Observe that if the good agents of $\Gamma$ start the execution of $\cmp(n)$ while the good agents of $\mathcal{Y}$ are executing $\swD(d,n)$, then $y'$, the group of at least $\mathcal{F}_{\max}+1$ good agents of $\Gamma$ which performs $EXPLO(n)$ during the execution of $\cmp(n)$, necessary meets a group of at least {$4\mathcal{F}_{\max}+2$} agents executing $\swD$ with the same parameters. Indeed, the beginning of $\swD(d,n)$ consists in waiting at least $d$ rounds (refer to section \ref{sec:block}), and {since every good agent spends exactly $2T(EXPLO(n))+2$ rounds executing $\cmp(n)$}, in view of the definition of $d$ the good agents of $\mathcal{Y}$ start $\swD(d,n)$ at some round in $\{t-d+1,\ldots,t\}$. Hence, in view of the definition of $t$, we know that every group of $\mathcal{W}$ executing $\swD$ with the same parameters that is encountered by $y'$, executes this routine with a first parameter that is $d$. Hence, each good agent of $y'$ has its variable $\mathcal{D}'=d$ by the end of the execution of $EXPLO(n)$. As a result, in view of the description of $\cmp(n)$, every good agent of $\Gamma$ has its variable $\mathcal{D}'=d$ at round $t$, which is a contradiction.

If the good agents of $\Gamma$ start the execution of $\cmp(n)$ while the good agents of $\mathcal{Y}$ are not executing $\swD(d,n)$, that implies no good agent starts to execute $\swD(d,n)$ by round $t$.
So, if the good agents of $y'$ meet no group of at least {$4\mathcal{F}_{\max}+2$} agents executing $\swD$ with the same parameters while performing $EXPLO(n)$ during the execution of $\cmp(n)$, then via similar arguments to those used in the second paragraph of this proof, we can show that every good agent of $\Gamma$ has its variable $\mathcal{D}'=d$ at round $t$. Otherwise, the good agents of $y'$ meet a group of of at least {$4\mathcal{F}_{\max}+2$} agents executing $\swD$ with the same parameter $d$ and $n$, while performing $EXPLO(n)$ during the execution of $\cmp(n)$, and similarly as in the above paragraph, we can also show that every good agent of $\Gamma$ has its variable $\mathcal{D}'=d$ at round $t$.

Hence, in all cases, we get a contradiction. Therefore, all the good agents belonging to any group of $\mathcal{W}$ discover $d$ and by Lemma~\ref{f:everyoneGroup}, the present lemma holds.

%$\mathcal{Y}$ as the agents of $\mathcal{Y}$ are idle on the node from which that started the execution of $\Syn(\mathcal{D})$ for at least $d$ rounds (refer to section \ref{sec:block}). Hence, all the good agents of $y'$ retrieve the correct value of $d$ and thus all the good agents of $\Lambda$ discover $d$ by the end of $\cmp(n)$. By contrast, if the good agents of $\Lambda$ starts the execution $\cmp(n)$ while the good agents of $\mathcal{Y}$ are also executing $\cmp(n)$, then from our previous discussion, we know that at least $\mathcal{F}_{\max}+1$ good agents of each group of $\mathcal{W}$ are idle on their nodes,  we can hence deduce that for each group of $\mathcal{W}$, $y'$ meet either all its good agents in \sta{\szJ} with the same indicator or at least $\mathcal{F}_{\max}+1$ of its good agents in state either \szK{} or \szL{}. Thus, all the good agents of $y'$ discover $d$ and which make all the good agents of $\Lambda$ discover $d$ by the end of $\cmp(n)$. This proves the lemma. 

 
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As mentioned at the beginning, throughout this section we assumed that $\mathcal{GK}=\lfloor\log \log f\rfloor$: we explicitely recall it in the statement of the following final result of this section.

\begin{theorem}\label{f:Theorem:main}

When $\mathcal{GK}=\lfloor\log \log f\rfloor$, Algorithm \ref{onlyf:algo:main} solves $f$-Byzantine gathering of $k$ good agents in a time polynomial in $n$ and $|l_{min}|$ if $k \geq 2 ((5f+1)(f+1)+1)$.
\end{theorem}

\begin{proof}

The proof of the theorem is made of two parts: the first part focuses on showing that there exists a round in which all the good agents declare the gathering on the same node while the second part shows that the gathering is declared within a time polynomial in $n$ and $|l_{min}|$.

\noindent \textbf{Part I}. From the description of the algorithm, Lemmas \ref{f:everyoneGroup} and \ref{lemma:cmp}, we know that every good agent starts the execution of $\swD(d,n)$ of line \ref{line:A} of algorithm \ref{onlyf:algo:main} with at least {$4\mathcal{F}_{\max}+1$} other good agents at the same round and from a same node at most $d$ rounds after the good agents of $\mathcal{Y}$.  By Theorem \ref{block2:proof:theo}, we know that all the good agent exit $\swD(d,n)$ in the same node and at the same round. That is, they all execute Line \ref{line:A+1} of algorithm \ref{onlyf:algo:main} in the same node and at the same round which completes the proof of Part I. 

\noindent \textbf{Part II}. From the description of the algorithm, we know that

\begin{equation}
  T(\tc(i))=\begin{cases}
      A(1) & $if$~ i=1 \\ 
       A(i)+ c (\sum\limits_{j=1}^{i-1} T(\tc(j)) &  $if$~ i>1
    \end{cases}
  \label{eq1}
\end{equation}

where {$c=76$ and $A(i)=T(\del_i)+120T(EXPLO(2^i))+24\mathcal{T}(i)-4$.}

We start by proving by induction on $i$ that 

\begin{equation}
\label{eq2}
T(\tc(i))= A(i) + c(\sum\limits_{j=0}^{i-2} A(i-j-1)(c+1)^{j}) ~ for ~ {i \geq 1}
\end{equation}



\indent \textit{\textbf{Base case}}. %When $i=3$, %
{When $i=1$, from equation \ref{eq1} we can deduce that \ref{eq2} is true for $i=1$.}

%\begin{tabular}{ll}
%$T(\tc(3))$ & $= A(3) + c (\sum\limits_{j=1}^{2} T(\tc(j))$\\
%%& $= A(3)+c (A(1)+ A(2)+c A(1))$\\
%& $= A(3) + c (A(2)+(c+1)A(1))$\\ 
%& $= A(3) + c(\sum\limits_{j=0}^{1} A(i-j-1)(c+1)^{j})$.   
%\end{tabular}

%We can deduce that (\ref{eq2}) is true for $i=3$.

\indent \textit{\textbf{Induction step}}. Let $i\geq 1$ be an integer. Suppose that (\ref{eq2}) is true for $i$. Then 

\begin{tabular}{ll}
$T(\tc(i+1))$  &  $= A(i+1)+ c (\sum\limits_{j=1}^{i} T(\tc(j))$ \\
             & $= A(i+1)+ c T(\tc(i))+ c(\sum\limits_{j=1}^{i-1} T(\tc(j))$\\
             & $= A(i+1)+ c T(\tc(i))+ T(\tc(i))- A(i)$ \\
     
             
             
\end{tabular}

By the induction hypothesis, we obtain: 

\begin{tabular}{ll}
$T(\tc(i+1))$ & $= A(i+1)+ (c+1) (A(i)+ c\sum\limits_{j=0}^{i-2} A(i-j-1)(c+1)^j)- A(i) $ \\
& $= A(i+1)+ c(\sum\limits_{j=0}^{i-1} A(i-j)(c+1)^j)$ \\
\end{tabular}

Thus, (\ref{eq2}) holds for $i+1$ which completes the proof of the induction step. 

By the induction principle, we can deduce that (\ref{eq2}) is true for any $i>2$. 

From Lemma \ref{f:lemma:group}, we know that at least {$4\mathcal{F}_{\max}+2$} good agents start the execution of $\sd$ by round $\beta=\Delta + \sum\limits_{j=1}^{s} T(\tc(s))$. We have shown that 

%\begin{tabular}{lll}
$\beta = \Delta+ A(s)+ c(\sum\limits_{j=0}^{s-2} A(i-j-1)(c+1)^j) <  \Delta + A(s)(1+ c\sum\limits_{j=0}^{s-2}(c+1)^j)= \Delta + A(s)(1+ c(\frac{(c+1)^{s-1}-1}{(c+1)-1}))$\\
%\end{tabular}

That is, $\beta <  \Delta + A(s)(1+ (c+1)^{s+1}) $. Remember that $s$ is the smallest positive integer such that $n \leq 2^s$ and $|l_{min}| \leq 2^s$. That is, $s= max(\lceil \log n \rceil, \lceil \log |l_{max}| \rceil)$. Remember also that $A(s)=T(\del_s)+480 T(EXPLO(2^s))+56 \mathcal{T}(s)-4$ where $\mathcal{T}(s)=4(2^sT(EXPLO(2^s)))^2+2T(EXPLO(2^s))$. Thus, we can deduce that the good agents of at least one group of at least $3\mathcal{F}_{\max}+2$ good agents starts the execution of $\sd$ within a time polynomial in $n$ and $|l_{\min}|$ from $\Delta$. 

{On another hand, as discussed in the proof of Lemma \ref{f:lemma:group}, we know that at round $\rho$ every good agent is awake and no good agent has started to execute $\tc(i+\lceil \log n\rceil+3)$. In view of the definition of $\mathcal{Y}$, $i \leq s$. Hence we can deduce that for any group of at least $3\mathcal{F}_{\max}+2$ good agent executing $\Syn(\mathcal{J})$, $\mathcal{J} \leq T(\sd(n))+ \sum\limits_{j=1}^{3s+3} T(\tc(j))$. Using the same arguments as above, we can show that $\mathcal{J}$ is polynomial in $n$ and $|l_{\min}|$ which implies that $d$ is also polynomial in $n$ and $|l_{\min}|$. }

{Since $\mathcal{J}$ is polynomial in $n$ and $|l_{\min}|$ and $\rho \leq \beta$, by Lemma \ref{f:everyoneGroup}, we know that in a time polynomial in  $n$ and $|l_{\min}|$ from $\Delta$, there exits a round from which every good agent starts the execution of $\cmp(n)$. Since every good agent spends the same number of rounds $x$ executing $\cmp(n)$ where $x$ is polynomial in $n$, by Lemma \ref{lemma:cmp}, we know that by round $\rho + \mathcal{D}_1+ 2T(EXPLO(n))+d+2$, every good agent is executing subroutine $\swD(\mathcal{D}',n)$ with $\mathcal{D}'=d$. By Theorem \ref{block2:proof:theo}, we can conclude that every good agent declares the gathering in a time polynomial in $n$ and $|l_{\min}|$ from $\Delta$ which completes the proof of Part II.}\\
 





From Part I and Part II, we can conclude that the theorem holds. 




 










%From lemma \ref{f:lemma:group}, we know that there exists $1 \leq i \leq s$ such that a group of at least $4\mathcal{F}_{max}+2$ good agents exit their execution of $\tc(i)$ with their respective $InGroup$ variable set to $true$ on the same node and at the same round $t \leq \Delta + \sum \limits_{j=1}^{s}T(\tc(j))$ at the latest. Recall that $s$ is the smallest positive integer such that $n \leq 2^s$ and $l_{min} \leq 2^s$. That is, $s= max(\lfloor \log n \rfloor, \lfloor \log l_{max} \rfloor)$. We can thus deduce that a group of at least $3\mathcal{F}_{max}+2$ agents starts the execution of $\sd$ in a time polynomial in $n$ and $l_{min}$ from round $\Delta$. Let $\mathcal{Y}$ and $t$ be the first group of at least $3\mathcal{F}_{max}+2$ agents that executes $\sd$ and the round in which the agents of $\mathcal{Y}$ start the execution of $\sd$. Recall that subroutine $\sd$ ends in a time polynomial in $n$ from $t$. At round $t+T(\sd)$ rounds, all the good agents $\mathcal{Y}$ are on the same node and all know the value of $n$. Moreover, every good agent is awake. Hence  for any pair of good agent $A$ and $B$, $delay_{(A,B)} \leq \mathcal{D}$. By lemma \ref{f:everyoneGroup}, at round $t+T(\sd)+\mathcal{D}$, every agent is in a group of at least $\mathcal{F}_{max}+2$ executing $\Syn(\mathcal{D})$ and having the same indicator and by Theorem \ref{xx} of section \ref{sec:block}, we can deduce that that all the good agents exit subroutine $\swD(\mathcal{D},n)$ on the same node and at the same round $t' \leq t+T(\sd)+\mathcal{D}+ T(\swD(\mathcal{D},n))$. Hence, we deduce that the theorem holds.
\end{proof}

